Improving Developers' Understanding of Regex Denial of Service Tools through Anti-Patterns and Fix Strategies

Regular expressions are used for diverse purposes, including input validation and firewalls. Unfortunately, they can also lead to a security vulnerability called ReDoS (Regular Expression Denial of Service), caused by a super-linear worst-case execution time during regex matching. Due to the severity and prevalence of ReDoS, past work proposed automatic tools to detect and fix regexes. Although these tools were evaluated in automatic experiments, their usability has not yet been studied; usability has not been a focus of prior work. Our insight is that the usability of existing tools to detect and fix regexes will improve if we complement them with anti-patterns and fix strategies of vulnerable regexes. We developed novel anti-patterns for vulnerable regexes, and a collection of fix strategies to fix them. We derived our anti-patterns and fix strategies from a novel theory of regex infinite ambiguity - a necessary condition for regexes vulnerable to ReDoS. We proved the soundness and completeness of our theory. We evaluated the effectiveness of our anti-patterns, both in an automatic experiment and when applied manually. Then, we evaluated how much our anti-patterns and fix strategies improve developers' understanding of the outcome of detection and fixing tools. Our evaluation found that our anti-patterns were effective over a large dataset of regexes (N=209,188): 100% precision and 99% recall, improving the state of the art 50% precision and 87% recall. Our anti-patterns were also more effective than the state of the art when applied manually (N=20): 100% developers applied them effectively vs. 50% for the state of the art. Finally, our anti-patterns and fix strategies increased developers' understanding using automatic tools (N=9): from median "Very weakly" to median "Strongly" when detecting vulnerabilities, and from median "Very weakly" to median "Very strongly" when fixing them.

==> bg-old.tex <==
%!TEX root = main.tex

% \FS{@FS: Maybe simplify this section?}
%	Background (0.2 pages)
%		ReDOS
%		Super-linearity
%			Existing Superlinearity anti-patterns
%		Ambiguity
%			Existing Ambiguity anti-patterns
% \JD{To ponder: is it worth putting in a threat model / statement of context for this work? A threat model is not quite the right phrase to use here, but a reader might be looking for it since the work has security applications.}

% \JD{The subsections in this section are very short. If space is an issue, I think it would be OK to use a ``vertical whitespace + no indent + boldface'' heading-like macro instead, possibly known as ``myparagraph'' in this document}

%This section describes background concepts to our work.
This section provides background on regexes (\cref{section:Background:regex}) and \REDOS (\cref{section:Background:redos}), 
describes the impact of \REDOS in practice (\cref{section:Background:impact}), and 
discusses the threat model (\cref{section:Background:model}). 

\mysection{Regular Expressions (Regexes)}
\label{section:Background:regex}

%\JD{Missing an inline subsection here.}

\mysubsection{Regexes}
\label{section:background:regex:regexes}
%% What is it?
A regex is a compact descriptive format used to specify a language: \ie a set of strings.
%% Syntax
Given a finite alphabet of terminal symbols, $\Sigma$, and the metacharacters, `$|$', `$\cdot$', and `$*$', 
%`$($', and `$)$', 
the regex syntax is~\cite{Sipser2006AutomataTheory}:

\vspace{-10px}
%\[ R \rightarrow \phi\mathrel{|}\epsilon\mathrel{|} \sigma \mathrel{|} R_1{\mlq|\mrq}R_2 \mathrel{|} R_1\cdot R_2 \mathrel{|} R_1\ast \]
\[ R \rightarrow \phi \;\Big{|}\; \epsilon \;\Big{|}\; \sigma \;\Big{|}\; R_1{|}R_2 \;\Big{|}\; R_1{\cdot}R_2 \;\Big{|}\; R_1* \]

%\JD{We are inconsistent about putting ` ' around metacharacters. I think it would be nicer to simply use a different (larger) vertical bar for the breaks between grammar destinations.}

%\JD{Use $R_1$ and $R_2$ if you need to include multiple Rs in a given line.}
%\AH{That would be better for readability. But to ensure recursiveness, i think we need to use the same R inside too.}
% \JD{Use a center dot instead of the period for concatenation. Is it cdot?}

\noindent
where $\phi$ denotes the empty language; 
$\epsilon$ is the empty string; 
the characters $\sigma \in \Sigma$ are terminal symbols;
$R_1|R_2$ is alternation (union); % of the languages of $R_1$ and $R_2$;
$R_1{\cdot}R_2$ is concatenation; % of the languages  of $R_1$ and $R_2$; and 
and
$R\ast$ is zero or more repetition (Kleene closure~\cite{kleene1951representation}).
%%
The language function $L:R\rightarrow 2^{\Sigma^\ast}$ gives semantics:

\begin{table}[h]
\vspace{-5px}
\centering
{
\normalsize
\begin{tabular}{ll}
$L(\phi) = \phi$                & 
$L(R_1|R_2) = L(R_1) \cup L(R_2)$   \\
$L(\epsilon) = \{\epsilon\}$    &
$L(R_1{\cdot}R_2) = L(R_1){\cdot}L(R_2)$   \\
$L(\sigma) = \{\sigma\}$        &
$L(R\ast) = L(R)\ast$          
\end{tabular}
}
\vspace{-5px}
\end{table}

%\begin{align*}
%L(\phi) &= \phi \\
%L(\epsilon) &= {\epsilon} \\ 
%L(\sigma) &= {\sigma} \\
%L(R1|R2) &= L(R1) \cup L(R2) \\
%L(R1R2) &= L(R1) \cdot L(R2) \\
%L(R\ast) &= L(R)\ast \\
%\end{align*}

%\JD{Lots of space being used here. I suggest a tabular layout, 2 rows with 3 columns.}
%\DY{I added more examples below to explicitly enumerate some syntactic sugar extensions we support.}
We refer to the above ``regular'' regexes, including alternation, concatenation, repetition, and ``syntactic sugar'' extensions, as (Kleene's) K-regexes.
These ``syntactic sugar'' extensions include 
  %any character `.' (as $\Sigma$); 
  character ranges \verb<[a-c]< (equivalent to \verb<a|b|c<);
  optional regex \verb<R?< (as \verb<R|<$\epsilon$);
  and
  various forms of repetition such as \verb<R+< (equivalent to \verb<RR*<) 
  and \verb<R{2,3}< (equivalent to \verb<RR|RRR<).
%various ($n$, $n$-or-more, $n$-to-$m$) repetitions \verb<{n}<, \verb<{n,}<, and \verb<{n,m}<;
%(where, for instance, \verb<{2,3}< corresponds to \verb<(RRR|RR)<; 
%%

%\FS{Extended the two paragraphs below to incorporate feedback from RA-Q2 in our rebuttal. Please, review.}
%\DY{I made minor edits: dropping K-regexes, LKA, BKR, 10\% etc.}
%\DY{Defined K-regexes above. We support K-regexes. We exclude non-regular features and extended character classes.}
%\JD{This seems like a strange place to talk about our implementation and compare to other \REDOS tools (recall, we have not even introduced \REDOS yet!). In the Background, can we focus on defining terms?}
%\FS{I tried to fix this. Please, review.}
%\DY{Reviewed. Comments removed.}

% \emph{Non-regular} features are more semantically complex.
% There are more semantically complex \emph{non-regular} regex features.
Outside the scope of K-regexes, there are also non-regular features.
The most commonly supported non-regular features are lookaround assertions, %(LKA, LKB, NLKA, NLKB), 
backreferences, %(BKR), 
atomic groups, and possessive quantifiers~\cite{Friedl2002MasteringRegexes}. 
These are semantically complex and their use is rare~\cite{Chapman2016RegexUsageInPythonApps,Davis2019RegexGeneralizability}.
%---they appear in only a minority (10\%) of real-world regexes \cite{Davis2019LinguaFranca}.
%
Our theory and anti-patterns therefore support K-regexes but currently exclude non-regular features.


\mysubsection{Regex Ambiguity}
The regex language semantics allow membership to be checked using a parser.
A regex is \emph{ambiguous} if there is a string in its language that can be matched with more than one parse tree \cite{brabrand2010typed,Sulzmann2017DerivAmbig}.
For example, the regex \verb<a|a< can parse the input ``\emph{a}'' in two ways,
\ie yielding two parse trees, one using the left \verb<a< and one the right.
%%

For K-regexes,
a regex match can be equivalently performed by simulating an input on a non-deterministic finite automaton (NFA) constructed from the regex (\eg using Thompson's algorithm~\cite{Thompson1968LinearRegexAlgorithm}).
%\JD{The preceding sentence is only true because we restricted the features to regular ones. Not sure how I feel about that.}
%%
%\AH{Added the sentence below to address the comment ``Are $\epsilon$ loops possible in the automata?'' Please, review}
%\DY{@AH, I moved/revised the $\epsilon$-free discussion here.}
To simplify discussion, we will reason about regex ambiguity over an equivalent, ambiguity-preserving, $\epsilon$-free NFA~\cite{weber1991degree,Weideman2017StaticExpressions} (with no $\epsilon$-loops).
%%
From the NFA perspective, a regex's NFA is ambiguous if there is a string that can be accepted along multiple paths of the NFA. %, \ie a non-deterministic choice exists and multiple choices lead to the accept state. % exists more than one ``path'' in the NFA in which an input can start from the initial node and reach one of the matching nodes.
%%
%For another regex \verb<(a|a)*<, an input ``$aaa...a$'' can be matched in ``many'' different ways.

\mysubsection{Infinitely Ambiguous (IA) Regex}
\label{sec:definition-ia-regex}
%\DY{If we want to explicitly distinguish SL and IA regexes (which I don't think necessary), then I think it would be useful to bring up an IA-but-not-SL example: e.g., a*a*.*}
%\DY{I think we should define ``ambiguity'' here: \eg multiple matching paths during NFA simulation, backtracking, explore all before declare a mismatch, etc., In the later note, I also suggested to introduce EDA and IDAd patterns/figures here.}
%\JD{The next sentence says ``IA'' before we have defined it in the prose (which we do shortly afterward). Typo?}
%%%
%A regex is infinitely ambiguous if it has an \emph{infinitely ambiguous (IA)} section~\cite{weber1991degree}.
%Thus, all SL regexes are IA regexes.
%An infinitely ambiguous (IA) regex shows an \emph{infinite-degree-of-ambiguity (IDA)}. Given an $\epsilon$-free finite automaton A, theorists~\cite{weber1991degree} have identified the necessary and sufficient conditions for A to be polynomially ambiguous($IDA_d$) or exponentially ambiguous(EDA). A polynomially (exponentially) ambiguous NFA has polynomially (exponentially) many paths(for ambiguity-preserving NFA constructions, \eg Thompson's~\cite{Thompson1968LinearRegexAlgorithm}). We assume the all the NFAs to be $\epsilon$-edge free by Weideman's~\cite{Weideman2017StaticExpressions} post processing.
Regexes can have various degrees of ambiguity:
  no ambiguity (deterministic);
  finitely ambiguous (bounded ambiguity regardless of input length);
  or
  infinitely ambiguous (polynomial or exponential) in the length of the input~\cite{allauzen2008general,stearns1985equivalence}.
A regex is infinitely ambiguous if it has a sub-regex (equivalently, an NFA section) 
with the \emph{infinite-degree-of-ambiguity (IDA)} property~\cite{weber1991degree}.
Given an $\epsilon$-free finite automaton A, the necessary and sufficient conditions for A to be infinitely ambiguous
%--- polynomially (PDA, also named $IDA_d$) or exponentially (EDA) ---
are given by Weber \& Seidl~\cite{weber1991degree}. 
Next we summarize these conditions.
%\AH{Added the sentence below to address the comment ``Are $\epsilon$ loops possible in the automata?'' Please, review}
%In this work, we assume all finite automata to be $\epsilon$-free.
%\DY{@AH, I moved the $\epsilon$-free discussion to the above Regex Ambiguity/NFA sub-section.}

%%% PDA
\cref{fig:ida}(a) illustrates how a \emph{polynomially IDA (PDA)} section appears in the NFA of a polynomially ambiguous regex.
A substring $label(\pi_i)$ can be matched in the loop $\pi_1$ at node $p$, the path $\pi_2$ from $p$ to $q$, or another loop $\pi_3$ at $q$.
For example, consider the regex \verb<a*a*< for an input ``$aa...a$'' of length $N$.
%\JD{Hmm, I believe that since we get to choose one partition then there are just $N$ matching paths. Since we might backtrack, each of those paths costs $\mathcal{O}(N)$ which is where the polynomial time complexity comes from.}
As any two partitions of the input can be matched with the first \verb<a*< and second \verb<a*<, there are $N$ matching paths.
Each of those paths costs $\mathcal{O}(N)$, so the total time complexity is quadratic in the size of input $\mathcal{O}(N^2)$.
%Thus the total number of matching paths could be $N + (N-1) + (N-2) + ... + 1 \approx N^2$. %: \ie the regex is polynomially ambiguous.

%%% EDA
%On the other hand,
\cref{fig:ida}(b) illustrates an \emph{exponentially IDA (EDA)} section in the NFA of an exponentially ambiguous regex.
A substring $label(\pi_i)$ can be matched in either of two loops $\pi_1$ or $\pi_2$ at node $p$.
The regex \verb<(a|a)*< is a representative example of exponentially ambiguous regexes.
Each `$a$' of the input ``$a...a$'' can be matched by either the upper or lower loop, and thus 
the total number of matching paths becomes $2^N$, leading to an exponential time complexity $\mathcal{O}(2^N)$.

\begin{figure}[t] 
    
    \centering 
    \begin{minipage}[b]{0.61\columnwidth}
      \centering
      \begin{tikzpicture}[baseline=-1.80em,initial text=]
        \tikzstyle{every state}=[inner sep=1pt, minimum size=0.2cm]
        
        \node[state] (q0) {$...$};
        \node[state, right = 0.4cm of q0] (q1) {$p$}; 
        \draw [->] (q0) edge node [above] {$...$} (q1);
        \draw (q1) edge[loop above] node [left] {\tt $\pi_1$} (q1);
        \node[state, right = 0.4cm of q1] (q2) {$q$}; 
        \draw [->] (q1) edge node [above] {\tt $\pi_2$} (q2);
        \draw (q2) edge[loop below] node [left] {\tt $\pi_3$} (q2);
        \node[state, right = 0.4cm of q2] (q3) {$...$};
        \draw [->] (q2) edge node [above] {$...$} (q3);
        \node at (1,1) (nodeC) {label($\pi_1$) = label($\pi_2$) = label($\pi_3$)};
        
      \end{tikzpicture} 
      \vspace{-5px}
      \caption*{(a) PDA (or $IDA_d$)} 
    \end{minipage}
    \begin{minipage}[b]{0.37\columnwidth}
      \centering
      \begin{tikzpicture}[baseline=-1.80em,initial text=]
        \tikzstyle{every state}=[inner sep=1pt, minimum size=0.2cm]

        \node[state] (q0) {$...$};
        \node[state, right = 0.4cm of q0]     (q1) {$p$}; 
        \draw [->] (q0) edge node [above] {$...$} (q1);
        \draw (q1) edge[loop above] node [left] {\tt $\pi_1$} (q1);
        \draw (q1) edge[loop below] node [left] {\tt $\pi_2$} (q1);
        \node[state, right = 0.4cm of q1] (q2) {$...$}; 
        \draw [->] (q1) edge node [above] {$...$} (q2);
        \node at (1,1) (nodeC) {label($\pi_1$) = label($\pi_2$)};
        
      \end{tikzpicture} 
      \vspace{-10px}
      \caption*{(b) EDA} 
    \end{minipage} 
    \vspace{-5px}
    \caption{
        Illustration of Polynomial and Exponential Degree of Ambiguity (PDA, EDA) in the NFA~\cite{weber1991degree}.
        %\DY{Cosmetic: Can we make (a) and (b) aligned?}
    }
    \vspace{-10px}
    \label{fig:ida}
\end{figure}

\mysection{Regex-Based Denial of Service (\REDOS)}
\label{section:Background:redos}
\JD{Shortening suggestion: Since we are looking only at the ``super-linear regex'' part of REDOS, this section is a bit too detailed. I think that one paragraph plus a small figure would be sufficient.}
\JD{Shortening suggestion: Can we merge this subsection with the next one, with the subsection title of ``Threat Model for Regex Denial of Service''?}

%\JD{@DY. The existing section here is a bit muddled, needs to be split into overview and threat model.}
%\subsubsection{Overview}
%\subsubsection{Threat Model}
%\subsubsection{OLD CONTENT:}

%\mysubsection{\REDOS}
Regex-based Denial of Service (\REDOS)~\cite{davis2021using,Crosby2003REDOS} is a security vulnerability by which 
%\JD{Since the diversion is typically considered to be coming from a malicious input, should we use the term ``attacker'' explicitly? (cf. threat model question above). Perhaps ``an \emph{attacker} diverts a web services resources''? or more indirectly, ``a web services's computational resources \ul{are diverted}...''?} 
a web service's computational resources are diverted from legitimate client interactions into an expensive regex match, degrading its quality of service.
Following the presentation of Davis \etal~\cite{davis2021using},
\REDOS is caused by a combination of three Conditions:
\begin{enumerate}[label=(C\arabic*)]
\item a \emph{backtracking regex engine} used in evaluation, and
\item a \emph{super-linear (SL) regex}, applied to evaluate
% \item a \emph{infinitely ambiguous (IA) regex}, applied to evaluate
\item a \emph{malign input}.
\end{enumerate}

\mysubsection{Backtracking Regex Engine}
Most regex engines 
%\JD{As noted before I still think this list of regex engine citations feels weird. The Cox and Davis citations are the ones that actually demonstrate this claim. If you delete this comment I will stop bringing it up :-)}
(\eg versions of PHP, % \JD{missing a PHP citation}, 
Perl, %~\cite{PerlRegEngine},
JavaScript, % (Node.js)~\cite{JSRegEngine}, 
Java, %~\cite{JavaRegEngine},
Python, %~\cite{PythonRegEngine},
Ruby, %~\cite{RubyRegEngine}, and 
and
\CSharp) %~\cite{CSharpRegEngine})
use a backtracking search algorithm, \eg Spencer's~\cite{Spencer1994RegexEngine},
to determine whether an input is in the language described by a regex~\cite{Cox2007RegExBible,Davis2019LinguaFranca}. 
The typical implementation has good common-case performance but can be problematically slow in the worst case
 --- \eg when it evaluates a \emph{super-linear (SL) regex} 
 % --- \eg when it evaluates a \emph{infinitely ambiguous (IA) regex} 
with \emph{malign input}~\cite{Davis2018EcosystemREDOS,Crosby2003REDOS,Crosby2003AlgorithmicComplexityAttacks}.

\mysubsection{Super-linear (SL) Regex}
%A regex is SL if its NFA is formed by: a \emph{prefix} section, followed by an \emph{infinitely ambiguous (IA)} section, followed by a \emph{suffix} section~\cite{Wustholz2017Rexploiter}.
% A regex is SL if its NFA is formed by: 
An SL regex is an IA regex whose NFA has
  a \emph{prefix} section, followed by an IDA section (either PDA or EDA), followed by a \emph{suffix} section~\cite{Wustholz2017Rexploiter}.
The IDA section is the root cause of the regex's super-linear behavior.
The prefix must be considered to reach this IDA section, and the suffix must typically lead to a mismatch in order to trigger backtracking.
% An IA regex is a necesseary condition for an SL regex.

\iffalse %%%%%%% IGNORE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[ht] 
    \centering 
    \begin{minipage}[b]{0.38\columnwidth}
      \centering
      \begin{tikzpicture}[baseline=-1.80em,initial text=]
        \tikzstyle{every state}=[inner sep=1pt, minimum size=0.2cm]
        
        \node[state, initial] (q0) {$q_0$};
        \node[state, right = 0.4cm of q0]     (q1) {$q$}; 
        \draw [->] (q0) edge node [above] {\tt $\pi_p$} (q1);
        \draw (q1) edge[loop above] node [left] {\tt $\pi_1$} (q1);
        \node[state, right = 0.4cm of q1] (q2) {$q'$}; 
        \draw [->] (q1) edge node [above] {\tt $\pi_2$} (q2);
        \draw (q2) edge[loop above] node [left] {\tt $\pi_3$} (q2);
        \node[state, right = 0.4cm of q2] (q3) {$q_r$}; 
        \draw [->] (q2) edge node [above] {\tt $\pi_s$} (q3);
        \node at (1,1) (nodeC) {label($\pi_1$) = label($\pi_2$) = label($\pi_3$)};
      \end{tikzpicture} 
      \caption*{\hspace{0.50cm}(a) IDA} 
    \end{minipage}
    \begin{minipage}[b]{0.38\columnwidth}
      \centering
      \begin{tikzpicture}[baseline=-1.80em,initial text=]
        \tikzstyle{every state}=[inner sep=1pt, minimum size=0.2cm]

        \node[state, initial, initial distance=0.25cm, accepting]     (q1) {$p$}; 
        \draw (q1) edge[loop above] node [left] {\tt $a$} (q1);
        \node[state, right = 0.4cm of q1, accepting] (q2) {$q$}; 
        \draw [->] (q1) edge node [above] {\tt $a$} (q2);
        \draw (q2) edge[loop above] node [left] {\tt $a$} (q2);
      \end{tikzpicture} 
      \caption*{\hspace{0.45cm}(b) NFA of  $a*a*$} 
    \end{minipage} 
    \caption{Illustration of IDA in the NFA}
    \label{fig:ida}
\end{figure}

\begin{figure}[ht] 
    \centering 
    \begin{minipage}[b]{0.38\columnwidth}
      \centering
      \begin{tikzpicture}[baseline=-1.80em,initial text=]
        \tikzstyle{every state}=[inner sep=1pt, minimum size=0.2cm]
        
        \node[state, initial] (q0) {$q_0$};
        \node[state, right = 0.4cm of q0]     (q1) {$q$}; 
        \draw [->] (q0) edge node [above] {\tt $\pi_p$} (q1);
        \draw (q1) edge[loop above] node [left] {\tt $\pi_1$} (q1);
        \draw (q1) edge[loop below] node [left] {\tt $\pi_2$} (q1);
        \node[state, right = 0.4cm of q1] (q2) {$q_r$}; 
        \draw [->] (q1) edge node [above] {\tt $\pi_s$} (q2);
        \node at (1,1) (nodeC) {label($\pi_1$) = label($\pi_2$)};
      \end{tikzpicture} 
      \caption*{\hspace{0.50cm} (a) EDA} 
    \end{minipage} 
    \begin{minipage}[b]{0.38\columnwidth}
      \centering
      \begin{tikzpicture}[baseline=-1.80em,initial text=]
        \tikzstyle{every state}=[inner sep=1pt, minimum size=0.2cm]

        \node[state, initial, initial distance=0.25cm, accepting]     (q1) {$p$}; 
        \draw (q1) edge[loop above] node [left] {\tt $a$} (q1);
        \draw (q1) edge[loop below] node [left] {\tt $a$} (q1);
      \end{tikzpicture} 
      \caption*{\hspace{0.45cm}(b) NFA of $(a|a)*$} 
    \end{minipage}
    \caption{Illustration of EDA in the NFA}
    \label{fig:eda}
\end{figure}

\fi %%%%%%% IGNORE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\mysubsection{Malign Input}
A malign input triggers the super-linear behavior of an SL regex by driving the backtracking engine into evaluating a polynomially or exponentially large number of possible NFA paths, exhausting available resources. 
%%%
Following the structure of an SL regex, a malign input is composed of three sections: a \emph{prefix}, then a \emph{pump}, then a \emph{suffix}.
The \emph{prefix} brings the engine to the IDA section of the regex, the pump produces polynomially or exponentially many paths to explore, and the \emph{suffix} causes the engine to mismatch.
This drives the engine to backtrack through the many paths~\cite{Berglund2014REDOSTheory}.
%\ie to continue evaluating the \emph{pump} through the polynomially or exponentially long list of possible paths in the infinitely ambiguous states of the IDA section of the IA regex.
%%%

\mysubsection{SL vs. IA Regexes}
Infinite ambiguity is a necessary but insufficient condition for super-linear behavior. %, but
%an IA regex may not be SL.
For example, the regex \verb<(a*)*.*< is IA but not SL.
% (with EDA) 
Its final sub-regex \verb<.*< accepts any string, so no mismatch-triggering suffix exists. %possible to trigger a mismatch (backtracking).

%\JD{I think an automaton illustration would be more useful than a tabular one. That way we convey some intuition, not just performance numbers. The Overleaf for S\&P'21 has code for this.}
%\JD{Specifically, a picture would be nice. There is latex inline illustration code in the S\&P'21 paper if we want to use a variation here.}
%\FS{@Adnan, I pasted below the code in the S\&P'21 paper. Please, modify it to use a different example to illustrate \REDOS. (JD adds: This is so we avoid copyright complaints from IEEE, as well as the minor risk of de-anonymizing ourselves).}
%\DY{I think the two IDA NFA patterns (EDA::exp (a*)* and IDAd::poly a*a*) should be visualized in the 2.3 IA regex section. I assume later our proof rely on the fact that these two are only two (necessary and sufficient) conditions for IDA.}
%\JD{I agree with DY --- let's use the illustration earlier if possible.}

% Impact of REDOS
%\mysubsection{The Impact of \REDOS in Practice}
\mysection{The Impact of \REDOS in Practice}
\label{section:Background:impact}
\JD{Shortening suggestion: Keep the figure, but merge it with the previous subsection with a single-sentence reference.}

The impact of a slow regex varies depending on how it is used in a web service.
For example, the company Cloudflare used a regex as part of deep packet inspection.
When it deployed a quartic regex in 2019, its network routing servers spent all of their time on a regex match, effectively halting their CDN service~\cite{Cloudflare2019REDOSPostMortem}.
As another example, the popular Q\&A website Stack Overflow used a quadratic regex for modest server-side rendering.
When a long problematic post reached the homepage, access to the homepage took several seconds, causing their monitoring system to mark each of their backend servers inoperable in succession.
This reduced their load-balancing capacity, eventually leading to an outage~\cite{2016StackOverflowOutage}.

%Regexes are used for diverse purposes, making the \REDOS impact of a specific regex difficult to predict.
%The impact may vary over time as the context of a regex varies, as was the case at Stack Overflow --- they used an SL regex for rendering, this affected page load times, and those times were later interpreted as a signal of server health. %, amplifying the effect of that slow regex.

%\subsubsection{Incidence in Practice}

%\JD{This is a figure and some prose that could be helpful. No prior REDOS paper has provided a similar plot. I think the plot will be interesting to the security audience, \eg to highlight the fact that \REDOS is on the rise but is still (in absolute terms) a rare issue. If we include it, I suggest we put it next to the Cloudflare/SO examples, probably in a subsubsection titled ``\REDOS vulnerabilities in practice''. (Although the data is novel, I think the Background is still the right place to put a CVE chart.)}
%\JD{It would be nice to indicate here that Cloudflare is security-sensitive regex, while Stack Overflow is general-purpose regex that happened to have security implications because of the liveness checks in their system design.}


Beyond these well-publicized examples of \REDOS, we examined CVE data for another perspective on the impact of \REDOS in practice.
\cref{fig:REDOSOverTime} shows the increasing trend of \REDOS CVEs each year since 2010.

\begin{figure}[] 
	\centering
    \includegraphics[width=0.9\columnwidth]{figures/CVEData/ReDoS-CVEs}
    %\vspace{-5px}
    \captionof{figure}{
        CVEs due to \REDOS since 2010.
        \JD{Shortening suggestion: Delete the rest of this caption. I don't think the detail is necessary.}
        % \FS{Agreed. Done.}
        The data were obtained by a two-step process: a preliminary labeling of the CVE database using key words and phrases (\eg ``\REDOS'' or ``extremely long time'' with a reference to regular expressions), followed by a manual inspection for accuracy.
    }
    \label{fig:REDOSOverTime}
\end{figure}

%\JD{I do not like the next paragraph very much. The point we are trying to make is that ``Hmm, not tooooo many CVEs, but also it's on the rise''. I don't like the reliance on conjecture here.}
%\DY{I dropped most of the paragraph. Mentioned ``increasing trend'' in the above paragraph.}

%The data indicates an increase in \REDOS CVEs over time.
%We conjecture that this can be attributed to a greater practitioner awareness of \REDOS, rather than any change in practitioners' regex practices.
%In other words, we interpret the trend in~\cref{fig:REDOSOverTime} to indicate that many software systems contain as-yet-undiscovered \REDOS vulnerabilities.

% \JD{At present, the background section does a good job of covering \REDOS, but does not inform me about previous work on identifying SL properties --- notably, the Davis anti-patterns, and analyses that use (a) NFA analyses; (b) transducers; (c) Brzozowski derivatives; (d) (any other kinds?). The ``Proposed approach'' feels out of context as a result. Perhaps we should move the Related Work here, or move the relevant bits for our Background?}
% \DY{I also thought that in 2. Backgroun, we should discuss Brabrand’s ambiguity theory and its limitation as well. Are we planning to discuss it later in Section 4. Theory? }
% \FS{Add a bridge paragraph to connect the background to "our approach"}

\mysection{Threat Model}
\label{section:Background:model}

%\DY{A new threat model section. Please review.}
%\JD{I looked and made minor tweaks.}
%\DY{Ack'ed}

% State the threat model
We suppose the following threat model for \REDOS, aligned with the common use of regexes for input sanitization in web software~\cite{Chapman2016RegexUsageInPythonApps,Wustholz2017Rexploiter,Michael2019RegexesAreHard}.
The victim's regex engine uses a backtracking regex engine (\REDOS Condition 1),
which is common for many server-side programming languages.
The victim uses a regex to sanitize the untrusted input (Condition 2).
The attacker controls the input string (Condition 3).
%\DY{TODO: assumption}
The input string could be arbitrary long.
%Although the victim may bound the length of the input string~\cite{Davis2018EcosystemREDOS}, as did both Stack Overflow and Cloudflare, each processed user-controlled strings containing kilobytes of text.
Bounding its length from the server side is not effective~\cite{Davis2018EcosystemREDOS}.
Both Stack Overflow and Cloudflare cases processed user-controlled strings containing kilobytes of text.



























==> intro-jamie.tex <==
%!TEX root = main.tex

%%%
% 30K view
%%%
\DY{We may want to revisit the title later. Now I see some important keywords include: usability, understandability, regex modality, anti-pattern, and fix strategies.}
\JD{I agree. Since this is a second submission, perhaps we can put this request into the letter to the reviewers?}

Regular expressions (\emph{regexes}) are a common software engineering tool for text processing~\cite{Chapman2016RegexUsageInPythonApps,Davis2018EcosystemREDOS}.
Regexes are used across the system stack~\cite{Li2008REL,Gogte2016HARE,Chiticariu2011SystemT,efftinge2006oaw}, including in security tasks such as
  input validation~\cite{Balzarotti2008Saner,Wassermann2008XSS}
  and
  web application firewalls~\cite{ModSecurityWAFRuleset,ClamAVRegexRules}.
   %anti-virus~\cite{}).
%and for general-purpose tasks
%  (\eg text processing
%   and
%   syntax highlighting~\cite{}).
% problem
Unfortunately, regexes can themselves cause a security vulnerability because of the high worst-case time complexity of backtracking-based regex engine implementations.
This algorithmic complexity vulnerability is known as 
\emph{Regular Expression Denial of Service (\REDOS)}~\cite{Crosby2003REDOS,Roichman2009ReDoS}.
%is an algorithmic complexity vulnerability~\cite{Crosby2003AlgorithmicComplexityAttacks}, denying service by exhausting computational resources.
%In a \REDOS exploit, a regex with super-linear worst-case execution time is triggered during regex matching.
%\REDOS can affect software that uses an unsafe (\emph{backtracking}) regex engine to evaluate a problematic (\emph{super-linear}) regex on untrusted strings (such as user input).
% wide impact:
%Unsafe regex engines are common in practice, including the regex engines shipped in many popular programming languages, \eg Java, JavaScript, Ruby, and Python~\cite{Cox2007RegExBible,Davis2019LinguaFranca}. 
% serious problem
%Unsafe regex engines use a naive backtracking-based predictive parser, which 
%This hazardous infrastructure exposes many web services to \REDOS. %, \eg to manipulate untrusted client data.
For example, \REDOS caused service outages at Stack Overflow in 2016~\cite{2016StackOverflowOutage} and at Cloudflare in 2019~\cite{Cloudflare2019REDOSPostMortem}.
Researchers report hundreds of vulnerable regexes in the software supply chain~\cite{Davis2018EcosystemREDOS} and in live web services~\cite{Staicu2018REDOS,barlas2022REDOS}.

% \begin{figure}[] 
% 	\centering
%     \includegraphics[width=.95\linewidth]{figures/illustrations/swisscheese.pdf}
%     %\vspace{-5px}
%     \captionof{figure}{
%         The Swiss cheese model~\cite{reason1990contribution,reason2000human} (defense in depth) for \REDOS. 
%         Most existing techniques to address \REDOS-vulnerable regexes are applied during their maintenance or after their deployment.
%         Our work provides early prevention, avoiding the composition of vulnerable regexes in the first place.
%         %avoiding composition of vulnerable regex
%         %(
%         %theory and anti-patterns
%         %),
%         %coping with vulnerable regexes
%         %(
%         %detecting SL regexes,
%         %repairing SL regexes,
%         %recovering from REDOS 
%         %),
%         %changing the infrastructure 
%         %(
%         %changing the regex engine
%         %)
%         %}
%         % \DY{Figure updated.}
%     }
%     \label{fig:swisscheese}
% \end{figure}

% \iffalse
% \begin{table}[]
% \begin{tabular}{p{2.6cm}|p{2.55cm}|p{2.55cm}}
% \hline
% \textbf{Existing Techniques for the Composition Stage}     & \textbf{Existing Techniques for the Maintenance Stage}          & \textbf{Existing Techniques for the Deployment Stage}                          \\
% \hline
% \hline
% Unsound anti-patterns~\cite{Davis2018EcosystemREDOS} & Detection techniques~\cite{Berglund2014REDOSTheory,Weideman2016REDOSAmbiguity,Weideman2017StaticExpressions,Wustholz2017Rexploiter,liu21sp,Kirrage2013rxxr,Rathnayake2014rxxr2,Sugiyama2014RegexLinearityAnalysis,Sulzmann2017DerivAmbig,Shen2018ReScueGeneticRegexChecker} & Infrastructure defense techniques~\cite{Cox2010RE2Implementation,davis2021using,bai2021runtime}  \\
% \hline
% \textbf{This work}: sound and complete theory, and derived anti-patterns          & Repair techniques~\cite{VanDerMerwe2017EvilRegexesHarmless,codykenny17,li2020flashregex,claver2021regis}    &                                    \\
% \end{tabular}
% \caption{Most existing techniques to address \REDOS-vulnerable regexes are applied during their maintenance or after their deployment. 
% Our work provides early prevention, avoiding the composition of vulnerable regexes in the first place.}
% % \vspace{-.1in}
% \label{tab:existingWork}
% \end{table}


% \begin{table}[]
% \begin{tabular}{@{}lp{7cm}@{}}
% \toprule
% Stage       & Techniques \\ \hline
% Maintenance & Detection techniques~\cite{Berglund2014REDOSTheory,Weideman2016REDOSAmbiguity,Weideman2017StaticExpressions,Wustholz2017Rexploiter,liu21sp,Kirrage2013rxxr,Rathnayake2014rxxr2,Sugiyama2014RegexLinearityAnalysis,Sulzmann2017DerivAmbig,Shen2018ReScueGeneticRegexChecker} \\ \hline
%             & Repair techniques~\cite{VanDerMerwe2017EvilRegexesHarmless,codykenny17,li2020flashregex,claver2021regis} \\ \hline
% Deployment  & Infrastructure defense~\cite{VanDerMerwe2017EvilRegexesHarmless,codykenny17,li2020flashregex,claver2021regis} \\ \hline
% Composition & Unsound anti-patterns~\cite{Davis2018EcosystemREDOS} \\ \hline
% (This work) & sound and complete theory, and derived anti-patterns \\ \hline
% \end{tabular}
% \end{table}
% \fi

%%%
% Existing solutions
%%%

Given the severity and prevalence of \REDOS, researchers have proposed mechanisms to help software engineers detect and remove \REDOS vulnerabilities.
%(see Table~\ref{tab:existingWork}).
The majority of these works offer tools that automatically
% apply to the software maintenance stage ---to 
% focus on automatically 
identify~\cite{Berglund2014REDOSTheory,Weideman2016REDOSAmbiguity,Weideman2017StaticExpressions,Wustholz2017Rexploiter,liu21sp,Kirrage2013rxxr,Rathnayake2014rxxr2,Sugiyama2014RegexLinearityAnalysis,Sulzmann2017DerivAmbig,Shen2018ReScueGeneticRegexChecker}
or
repair~\cite{VanDerMerwe2017EvilRegexesHarmless,codykenny17,li2020flashregex,claver2021regis}
vulnerable regexes.
% --- or after software deployment~\cite{Cox2010RE2Implementation,davis2021using,bai2021runtime}.
% Others have considered transparent runtime mitigations~\cite{Cox2010RE2Implementation,bai2021runtime,davis2021using}.
\FS{I removed the mention of other mitigations above. I think it distracts from the main goal of the paper.}
However, although these works are shown to be effective on large regex datasets~\cite{Davis2018EcosystemREDOS,Davis2019RegexGeneralizability}, none of them examines the \emph{usability} of the proposed tools.
Developers often refuse automated tools with low usability, \eg 95\% of developers reject tools when they cannot understand the results~\cite{johnson2013don}. 

%%%
% Our approach
%%%
In this paper, we describe novel approaches designed for high user understandability when developers (1) identify and (2) repair vulnerable regexes.
Our approach follows the paradigm of \emph{anti-patterns} and \emph{repair strategies}.
Developers obtain high understanding when tools provide: 
examples, 
support to avoid repeating problems, and 
proposed fixes 
\cite{johnson2013don}.
Our goal is that developers will improve their understanding using: 
(1) our \emph{anti-patterns} as examples to understand what makes a vulnerable regex and 
to avoid composing them in the future; and 
(2) our \emph{repair strategies} as proposed fixes for their vulnerable regexes.
% We designed our anti-patterns and repair strategies to complement existing tools, and we expect developers to use them in combination.
% Our approach follows the paradigm of \emph{anti-patterns} and \emph{repair strategies}~\cite{XXX}, which have been successful in improving user understandability in other cybersecurity contexts~\cite{AAA,BBB,CCC}.
\FS{I commented out the sentence above, since I could not find studies of security anti-patterns that included usability or understanding.}

\iffalse
%%%
% Improving Existing solutions
%%%
Our approach differs from prior work in three ways.
First, we describe our anti-patterns in the modality of the regex language because this is the modality that most developers better understand~\cite{bai2019exploring}, as opposed to a finite automaton representation~\cite{Weideman2016REDOSAmbiguity,Wustholz2017Rexploiter}.
Second, unlike the existing regex-level anti-patterns~\cite{Davis2018EcosystemREDOS}, we ground our anti-patterns in a novel theoretical representation of \REDOS vulnerability.
\DY{TODO: Add a comment on repair strategies as well, depending on our claims on the soundness/completeness of fix strategies.}
\JD{Good point, let's see what we end up writing there.}
\FS{See my attempt in the sentence below.}
Third, our repair strategies support developers when repairing their own regexes, as opposed to repairing them automatically \eg \cite{VanDerMerwe2017EvilRegexesHarmless,li2020flashregex,claver2021regis} (which may make it harder for them to understand and trust the repair).
\fi


%%%
% Improving Existing solutions
%%%
\FS{I made a different attempt at the comparison with prior work (I disabled Jamie's one above). I would like to focus on prior work first (as opposed to ours), and to focus on claims that we can back up with our experiments.}
Our approach differs from prior work in three ways.
First, compared to existing automatic tools to identify~\cite{Berglund2014REDOSTheory,Weideman2016REDOSAmbiguity,Weideman2017StaticExpressions,Wustholz2017Rexploiter,liu21sp,Kirrage2013rxxr,Rathnayake2014rxxr2,Sugiyama2014RegexLinearityAnalysis,Sulzmann2017DerivAmbig,Shen2018ReScueGeneticRegexChecker} and repair~\cite{VanDerMerwe2017EvilRegexesHarmless,codykenny17,li2020flashregex,claver2021regis} vulnerable regexes, 
our approach complements them to increase result understanding.
We expect developers to use both approaches in combination.
Second, compared to the finite-automaton-based patterns~\cite{Weideman2016REDOSAmbiguity,Wustholz2017Rexploiter} that existing tools use to automatically identify vulnerable regexes, 
our anti-patterns use the modality of the regex language.
This is the modality that most developers better (or only) understand~\cite{bai2019exploring,wang2019exploring}.
\FS{Reminder: double-check these two references above.}
Third, compared to existing regex-modality anti-patterns~\cite{Davis2018EcosystemREDOS}, 
we ground ours in our novel theoretical representation of \REDOS vulnerability.
We expect this to provide high precision and recall.



%%%
% Evaluation
%%%
In our evaluation, we found that our proposed anti-patterns and repair strategies complement existing automated techniques to identify and fix regexes vulnerable to \REDOS.
There are three main results.
First, we proved the soundness and completeness of our underlying theory of regex infinite ambiguity (IA) ---a necessary component of \REDOS. (\cref{section:Theory,section:Appendix-Proofs}).
Second, %to evaluate our derived anti-patterns (\cref{section:AntiPatterns}), we performed two complementary experiments (\cref{section:Experiment1}, \cref{sec:Experiment2}, and \cref{sec:Experiment3}).
our anti-patterns provide higher precision and recall than existing anti-patterns in the regex modality --- 100\% vs. 50\% precision, and 99\% vs. 87\% recall~\cref{section:Experiment1}.
Third, in a user study (\TODO{N=X})~\cref{sec:Experiment3},
  we found that open-source software developers generally preferred the results of our anti-patterns and repair strategies in addition to the output of the automated tools when analyzing and repairing \REDOS vulnerabilities in their software, \eg noting
%   ``\emph{I do understand the problem with the earlier one (with anti-patterns) and this one (repaired with fix strategies) does not have the problem, I can explain it out loud with the anti-patterns so I do understand it.}''.
  ``\emph{The output of the tool(detection) should mention the anti-pattern that plays a role in the detected vulnerability. In simple cases the automatic repair might be acceptable. In others, human engineering might be the better approach/choice}''.
  \JD{@Adnan can we use a quote that makes an explicit comparison between our approach and the existing tools?}
  \AH{Replaced the quote. Please check.}
  \FS{@Adnan do we have a quote that is more descriptive (\eg ``the anti-patterns help me understand'') as opposed to prescriptive (``the tool should mention the anti-patterns'')?}
  \DY{Need discussion. I don't think the current quote strongly supports our story.}
  \JD{Agree.}

%%%
% Summary of contributions
%%%

% contributions
In summary, this paper provides the following contributions:
\begin{enumerate}
	\item A sound, complete theory of regex infinite ambiguity (IA) (\cref{section:Theory}).
	\item Anti-patterns, derived from our theory, that developers can apply to identify vulnerable regexes (\cref{section:AntiPatterns}).
	Accompanying repair strategies to repair vulnerable regexes (\cref{section:FixPatterns}).
	\item A quantitative evaluation of the comprehensiveness of our proposed anti-patterns over a large-scale of real-world regexes, showing that they capture the wide majority of IA regexes (\cref{section:Experiment1}).
	\item A human-subjects evaluation of the usability of our proposed approach, showing that our approach gave developers greater understanding than existing approaches when detecting and repairing \REDOS regexes (\cref{sec:Experiment3}).
	%\item A second human-subjects evaluation, showing that our IA anti-patterns and fix patterns consistently provided higher understanding of what makes regexes vulnerable and what makes repaired regexes not vulnerable than when developers applied only existing tools (\cref{sec:Experiment3}).
\end{enumerate}
































% \begin{figure}[ht] 
%     \centering 
%     \begin{minipage}[b]{0.18\columnwidth}
%       \centering
%       \begin{tikzpicture}[baseline=-1.80em,initial text=]
%         %[initial text=]
%         \tikzstyle{every state}=[inner sep=0pt, minimum size=0.2cm]

%         \node[state, initial, initial distance=0.25cm]     (q1) {$$}; 
%         \node[state, right = 0.4cm of q1, accepting] (q2) {$$}; 
%         %\node[state, right of=q2, accepting] (q3) {$$}; 
%         \draw [->] (q1) edge node [above] {\tt $a$} (q2);
%         %\draw [->] (q2) edge node [above] {\tt $b$} (q3);
%       \end{tikzpicture} 
%       \caption*{\hspace{0.5cm}$a$}
%     \end{minipage} 
%     \begin{minipage}[b]{0.18\columnwidth}
%       \centering
%       \begin{tikzpicture}[baseline=-1.80em,initial text=]
%         \tikzstyle{every state}=[inner sep=0pt, minimum size=0.2cm]

%         \node[state, initial, initial distance=0.25cm]     (q1) {$$}; 
%         \node[state, above = 0.3cm of q1] (q2) {$$}; 
%         \node[state, right = 0.3cm of q1, accepting] (q3) {$$}; 
%         \draw [->] (q1) edge node [left] {\tt $a$} (q2);
%         \draw [->] (q2) edge node [above, pos=0.75] {\tt $b$} (q3);
%       \end{tikzpicture} 
%       \caption*{\hspace{0.5cm}$a \cdot b$}
%     \end{minipage} 
%     \begin{minipage}[b]{0.18\columnwidth}
%       \centering
%       \begin{tikzpicture}[baseline=-1.80em,initial text=]
%         \tikzstyle{every state}=[inner sep=0pt, minimum size=0.2cm]

%         \node[state, initial, initial distance=0.25cm]     (q1) {$$}; 
%         \draw (q1) edge[loop above] node [left] {\tt $a$} (q1);
%         \node[state, right = 0.4cm of q1, accepting] (q2) {$$}; 
%         \draw [->] (q1) edge node [above] {\tt $\epsilon$} (q2);
%       \end{tikzpicture} 
%       \caption*{\hspace{0.45cm}$a*$}
%     \end{minipage} 
%     \begin{minipage}[b]{0.18\columnwidth}
%       \centering
%       \begin{tikzpicture}[baseline=0em,initial text=]
%         \tikzstyle{every state}=[inner sep=0pt, minimum size=0.2cm]

%         \node[state, initial, initial distance=0.25cm]     (q1) {$$}; 
%         \node[state, above right = 0.4cm of q1]     (q2) {$$}; 
%         \node[state, below right = 0.4cm of q1]     (q3) {$$}; 
%         \node[state, below right = 0.4cm of q2, accepting]     (q4) {$$}; 
%         \draw [->] (q1) edge node [above, pos=0.25] {\tt $\epsilon$} (q2);
%         \draw [->] (q1) edge node [below, pos=0.25] {\tt $\epsilon$} (q3);
%         \draw [->] (q2) edge node [above, pos=0.75] {\tt $a$} (q4);
%         \draw [->] (q3) edge node [below, pos=0.75] {\tt $b$} (q4);
%       \end{tikzpicture} 
%       \caption*{\hspace{0.6cm}$a \vert b$}
%     \end{minipage} 
%     \hspace{0.02\columnwidth}
%     \vline
%     %\hspace{0.01\columnwidth}
%     \begin{minipage}[b]{0.18\columnwidth}
%       \centering
%       \tikzset{invisible/.style={minimum width=0mm,inner sep=0mm,outer sep=0mm}}
%       \begin{tikzpicture}%[baseline=(current bounding box.north)]
%         [initial text=]
%         \tikzstyle{every state}=[inner sep=0pt, minimum size=0.2cm]

%         % \node[state, initial]     (q1) {$$}; 
%         % \node[state, right of=q1, accepting] (q2) {$$}; 
%         % %\node[state, right of=q2, accepting] (q3) {$$}; 
%         % \draw [->] (q1) edge node [above] {\tt $a$} (q2);
%         % %\draw [->] (q2) edge node [above] {\tt $b$} (q3);

%         \node[state, initial, initial distance=0.25cm] (q1) {$$};
%         %\node[state, right = of q1] (q2) {$q_2$};
%         \node[state, above right = 0.4cm of q1] (q2) {$$};
%         \node[state, below right = 0.4cm of q1] (q3) {$$};
%         \node[state, below right = 0.4cm of q2, accepting] (q4) {$$};

%         \draw[->] (q1) edge [] node [above, pos=0.25] {\tt $\epsilon$} (q2);
%         \draw[->] (q1) edge [] node [below, pos=0.25] {\tt $\epsilon$} (q3);
%         \draw[->] (q2) edge [] node [above, pos=0.75] {\tt $a$} (q4);
%         \draw[->] (q3) edge [] node [below, pos=0.75] {\tt $a$} (q4);

%         \node[label=left:{$\epsilon$}, above= 0.47cm of q1,invisible] (above1) {};
%         \draw (q4) |- (above1);
%         \draw[->] (above1) -- (q1);
%       \end{tikzpicture} 
%       \caption*{\hspace{0.7cm}$(a \vert a)$+}
%     \end{minipage}
%     % \caption{
%     %     \KREsAcro operators and NFA equivalents for character, concatenation, repetition, and disjunction.
%     %     NFAs for \KREsAcros have in-degree and out-degree $\leq 2$, although this is higher under $\epsilon$-closure.
%     %     The final figure shows an exponentially ambiguous \KREsAcro.
%     % }
%     \label{figure:regex2NFA} 
% \end{figure} 

% \begin{table}
%     % DECREASE FONT SIZE?
%     %\scriptsize
%     %\footnotesize
%     %\small
%     \centering
%     \caption{
%       Regexes, time complexity, and the length of problematic input $|w|$ that necessitates a 10-second regex match in \TODO{Java-OpenJDK-X.XX}.
%       Each of these exhibits slow behavior on the input ``a$\stackrel{n}{\cdots}$ab''.
%       Machine is desktop class (\TODO{CPU specs go here}).
%     }
%     \begin{tabular} {cccc}
%     \toprule
%     \textbf{Regex}  & \textbf{Complexity}   & \textbf{$|w|$} \\
%     \toprule
%     \verb<^a*a*$<   & $\mathcal{O}(|w|^2)$  & ? \\
%     \verb<^a*a*a*$< & $\mathcal{O}(|w|^3)$  & ? \\
%     \verb<^(a|a)*$< & $\mathcal{O}(2^{|w|})$ & ? \\
%     \verb<^(a*)*$<  & $\mathcal{O}(2^{|w|})$ & ? \\
%     \bottomrule
%     \label{table:RegexQueryResponseTiming}
%     \end{tabular}
%     \vspace{-0.30cm}
% \end{table} 



==> intro-new-separate-contributions.tex <==
%!TEX root = main.tex

%%%
% 30K view
%%%
\DY{We may want to revisit the title later. Now I see some important keywords include: usability, understandability, regex modality, anti-pattern, and fix strategies.}
\JD{I agree. Since this is a second submission, perhaps we can put this request into the letter to the reviewers?}

Regular expressions (\emph{regexes}) are a common software engineering tool for text processing~\cite{Chapman2016RegexUsageInPythonApps,Davis2018EcosystemREDOS}.
Regexes are used across the system stack~\cite{Li2008REL,Gogte2016HARE,Chiticariu2011SystemT,efftinge2006oaw}, including in security tasks such as
  input validation~\cite{Balzarotti2008Saner,Wassermann2008XSS}
  and
  web application firewalls~\cite{ModSecurityWAFRuleset,ClamAVRegexRules}.
   %anti-virus~\cite{}).
%and for general-purpose tasks
%  (\eg text processing
%   and
%   syntax highlighting~\cite{}).
% problem
Unfortunately, regexes can themselves cause a security vulnerability because of the high worst-case time complexity of backtracking-based regex engine implementations.
This algorithmic complexity vulnerability is known as 
\emph{Regular Expression Denial of Service (\REDOS)}~\cite{Crosby2003REDOS,Roichman2009ReDoS}.
%is an algorithmic complexity vulnerability~\cite{Crosby2003AlgorithmicComplexityAttacks}, denying service by exhausting computational resources.
%In a \REDOS exploit, a regex with super-linear worst-case execution time is triggered during regex matching.
%\REDOS can affect software that uses an unsafe (\emph{backtracking}) regex engine to evaluate a problematic (\emph{super-linear}) regex on untrusted strings (such as user input).
% wide impact:
%Unsafe regex engines are common in practice, including the regex engines shipped in many popular programming languages, \eg Java, JavaScript, Ruby, and Python~\cite{Cox2007RegExBible,Davis2019LinguaFranca}. 
% serious problem
%Unsafe regex engines use a naive backtracking-based predictive parser, which 
%This hazardous infrastructure exposes many web services to \REDOS. %, \eg to manipulate untrusted client data.
For example, \REDOS caused service outages at Stack Overflow in 2016~\cite{2016StackOverflowOutage} and at Cloudflare in 2019~\cite{Cloudflare2019REDOSPostMortem}.
Researchers report hundreds of vulnerable regexes in the software supply chain~\cite{Davis2018EcosystemREDOS} and in live web services~\cite{Staicu2018REDOS,barlas2022REDOS}.

% \begin{figure}[] 
% 	\centering
%     \includegraphics[width=.95\linewidth]{figures/illustrations/swisscheese.pdf}
%     %\vspace{-5px}
%     \captionof{figure}{
%         The Swiss cheese model~\cite{reason1990contribution,reason2000human} (defense in depth) for \REDOS. 
%         Most existing techniques to address \REDOS-vulnerable regexes are applied during their maintenance or after their deployment.
%         Our work provides early prevention, avoiding the composition of vulnerable regexes in the first place.
%         %avoiding composition of vulnerable regex
%         %(
%         %theory and anti-patterns
%         %),
%         %coping with vulnerable regexes
%         %(
%         %detecting SL regexes,
%         %repairing SL regexes,
%         %recovering from REDOS 
%         %),
%         %changing the infrastructure 
%         %(
%         %changing the regex engine
%         %)
%         %}
%         % \DY{Figure updated.}
%     }
%     \label{fig:swisscheese}
% \end{figure}

% \iffalse
% \begin{table}[]
% \begin{tabular}{p{2.6cm}|p{2.55cm}|p{2.55cm}}
% \hline
% \textbf{Existing Techniques for the Composition Stage}     & \textbf{Existing Techniques for the Maintenance Stage}          & \textbf{Existing Techniques for the Deployment Stage}                          \\
% \hline
% \hline
% Unsound anti-patterns~\cite{Davis2018EcosystemREDOS} & Detection techniques~\cite{Berglund2014REDOSTheory,Weideman2016REDOSAmbiguity,Weideman2017StaticExpressions,Wustholz2017Rexploiter,liu21sp,Kirrage2013rxxr,Rathnayake2014rxxr2,Sugiyama2014RegexLinearityAnalysis,Sulzmann2017DerivAmbig,Shen2018ReScueGeneticRegexChecker} & Infrastructure defense techniques~\cite{Cox2010RE2Implementation,davis2021using,bai2021runtime}  \\
% \hline
% \textbf{This work}: sound and complete theory, and derived anti-patterns          & Repair techniques~\cite{VanDerMerwe2017EvilRegexesHarmless,codykenny17,li2020flashregex,claver2021regis}    &                                    \\
% \end{tabular}
% \caption{Most existing techniques to address \REDOS-vulnerable regexes are applied during their maintenance or after their deployment. 
% Our work provides early prevention, avoiding the composition of vulnerable regexes in the first place.}
% % \vspace{-.1in}
% \label{tab:existingWork}
% \end{table}


% \begin{table}[]
% \begin{tabular}{@{}lp{7cm}@{}}
% \toprule
% Stage       & Techniques \\ \hline
% Maintenance & Detection techniques~\cite{Berglund2014REDOSTheory,Weideman2016REDOSAmbiguity,Weideman2017StaticExpressions,Wustholz2017Rexploiter,liu21sp,Kirrage2013rxxr,Rathnayake2014rxxr2,Sugiyama2014RegexLinearityAnalysis,Sulzmann2017DerivAmbig,Shen2018ReScueGeneticRegexChecker} \\ \hline
%             & Repair techniques~\cite{VanDerMerwe2017EvilRegexesHarmless,codykenny17,li2020flashregex,claver2021regis} \\ \hline
% Deployment  & Infrastructure defense~\cite{VanDerMerwe2017EvilRegexesHarmless,codykenny17,li2020flashregex,claver2021regis} \\ \hline
% Composition & Unsound anti-patterns~\cite{Davis2018EcosystemREDOS} \\ \hline
% (This work) & sound and complete theory, and derived anti-patterns \\ \hline
% \end{tabular}
% \end{table}
% \fi

%%%
% Existing solutions
%%%

% Given the severity and prevalence of \REDOS, researchers have proposed mechanisms to help software engineers detect and remove \REDOS vulnerabilities.
% %(see Table~\ref{tab:existingWork}).
% The majority of these works offer tools that automatically
% % apply to the software maintenance stage ---to 
% % focus on automatically 
\HIDDEN{
    1 comprehensiveness of our characterization (as in past work)
    2 usability of our characterization
    3 effect of our characterization on tools usability
    4 effect of our repair strategies on repair tools usability
}

Given the severity and prevalence of \REDOS, 
researchers have developed
characterizations of regexes vulnerable to it, \eg~\cite{Weideman2016REDOSAmbiguity,Wustholz2017Rexploiter,Davis2018EcosystemREDOS},
and automatic tools to
identify them, \eg~\cite{Berglund2014REDOSTheory,Weideman2016REDOSAmbiguity,Weideman2017StaticExpressions,Wustholz2017Rexploiter,liu21sp,Kirrage2013rxxr,Rathnayake2014rxxr2,Sugiyama2014RegexLinearityAnalysis,Sulzmann2017DerivAmbig,Shen2018ReScueGeneticRegexChecker}.

These approaches have limitations.
Existing characterizations are either expressed as finite automata~\cite{Weideman2016REDOSAmbiguity,Wustholz2017Rexploiter} (but most developers better or only understand the modality of the regex language~\cite{bai2019exploring,wang2019exploring}) or provide very low precision~\cite{Davis2018EcosystemREDOS}.
Existing automated tools provided high effectiveness in automated experiments~\cite{Davis2018EcosystemREDOS,Davis2019RegexGeneralizability}, but no studies examined their \emph{usability} when applied by humans.
\FS{Double check this claim above.}
Developers often refuse automated tools with low usability, \eg 95\% of developers reject tools when they cannot understand the results~\cite{johnson2013don}. 

In this paper, we propose a novel characterization of regex infinite ambiguity (IA): IA anti-patterns.
The IA region of a regex is a necessary component of \REDOS.
It is also the region that developers fix when they repair vulnerable regexes~\cite{Davis2018EcosystemREDOS}.
\FS{Double check this claim above.}
We ground our anti-patterns in a novel theoretical representation of regex infinite ambiguity.
% \FS{Story 1: Experiment 2 is important. Anti-patters are for composition also. Experiment 2's goal was to find out if the anti-patterns were usable themselves. }
% The goal of our IA anti-patterns is twofold.
% First, to complement existing automated tools improving their usability, \ie their result understanding (since they may serve as examples and help to avoid repeating problems~\cite{johnson2013don}).
% Second, to also enable developers to identify IA when they decide not to use tools, \eg during regex composition if they disrupt their workflow \cite{johnson2013don}.
\FS{Story 2: Experiment 2 is not so important.}
The goal of our IA anti-patterns is to complement existing automated tools, improving their usability, \ie their result understanding (since they may serve as examples and help to avoid repeating problems~\cite{johnson2013don}).

We evaluate multiple aspects of our IA anti-patterns, formulating the following research questions:
\emph{(RQ1: Comprehensiveness) Do our IA anti-patterns characterize IA effectively in a large variety of regexes?}
\emph{(RQ2: Usability of anti-patterns) Are our IA anti-patterns usable enough for developers to characterize IA effectively?}
\emph{(RQ3: Usability of tools) Do our IA anti-patterns improve result understandability when using automatic tools to detect regexes vulnerable to \REDOS?}
To the extent of our knowledge, this is the first study to evaluate the usability of characterizations or tools to identify regexes vulnerable to \REDOS.
\FS{Does RQ2 feel out of place? I'm trying to reduce its importance by not mentioning it as a goal of our anti-patterns (in the paragraph above this one). I'm not sure I accomplish that well. 
The alternative would be to claim that our anti-patterns also have the goal to support developers in the absence of tools, but I think our reviewers already mentioned that our current experiment is not convincing to them. If we use this alternative framing, RQ2 makes more sense, but we would have to use a strong discussion of why the current numbers in experiment 2 are enough and generalizable.
Thoughts?}

% In our evaluation, our anti-patterns achieved these goals.
Our evaluation provided multiple findings.
For RQ1, we proved the soundness and completeness of our underlying theory of regex infinite ambiguity (\cref{section:Theory,section:Appendix-Proofs}).
We also further validated the proof with an experiment and found that our anti-patterns provided much higher effectiveness (100\% precision, 99\% recall) than existing anti-patterns in the regex modality~\cite{Davis2018EcosystemREDOS} (50\% precision, 87\% recall) when applied over a large-scale dataset of \AnalyzedNRegexes real-world regexes \cite{Davis2019LinguaFranca} (\cref{section:Experiment1}).
For RQ2, we found that even beginner and intermediate developers (100\% of \HumanSubjectsN studied) were able to effectively identify IA in regexes, in 5 different regex tasks, greatly improving over existing anti-patterns (50\%).
For RQ3, we found that open-source developers (\TODO{X\%} of \TODO{Y} studied) consistently improved their understanding of the results of a detection tool when they used our anti-patterns in combination with it.
They also consistently (\TODO{Z\%}) reported that they found them helpful and would continue using them in the future.
\FS{I'm not saying anything about RQ3 being more realistic than RQ2. Do we want to emphasize that aspect here?}

Once developers have identified that a regex is vulnerable to \REDOS and its IA region, they have to fix it.
Researchers have also proposed tools for this, \eg~\cite{VanDerMerwe2017EvilRegexesHarmless,codykenny17,li2020flashregex,claver2021regis}.
However, the \emph{usability} of these repair tools has also not been studied, and they may also be underused or rejected if they are not usable.

In this paper, we also provide a characterization of fix strategies to repair the IA region of a regex vulnerable to \REDOS.
We derived these fix strategies systematically from our anti-patterns and past characterizations of vulnerable regexes \cite{VanDerMerwe2017EvilRegexesHarmless}.
\FS{Double-check citation above.}
The goal of our IA fix strategies is to complement existing automated tools, improving their usability, since they may serve as proposed fixes~\cite{johnson2013don}.
% Third, our repair strategies support developers when repairing their own regexes, as opposed to repairing them automatically \eg \cite{VanDerMerwe2017EvilRegexesHarmless,li2020flashregex,claver2021regis} (which may make it harder for them to understand and trust the repair).

We evaluated our fix strategies formulating an additional research question:
\emph{(RQ4: Usability of tools) Do our IA fix strategies improve result understandability when using automatic tools to fix regexes vulnerable to \REDOS?}
To the extent of our knowledge, this is the first study to evaluate the usability of tools to repair regexes vulnerable to \REDOS.
\FS{Double-check this claim}
In our evaluation for RQ4, we found that 
open-source developers (\TODO{X\%} of \TODO{Y} studied) consistently improved their understanding of the resulting repaired regex when they used our fix strategies in combination with an automatic repair tool.
They also consistently (\TODO{Z\%}) reported that they found them helpful and would continue using them in the future.

%%%
% Summary of contributions
%%%

% contributions
\FS{TODO: These contributions need to be revisited, but everything above is done.}
In summary, this paper provides the following contributions:
\begin{enumerate}
	\item A sound, complete theory of regex infinite ambiguity (IA) (\cref{section:Theory}).
	\item Anti-patterns, derived from our theory, that developers can apply to identify vulnerable regexes (\cref{section:AntiPatterns}).
	Accompanying repair strategies to repair vulnerable regexes (\cref{section:FixPatterns}).
	\item A quantitative evaluation of the comprehensiveness of our proposed anti-patterns over a large-scale of real-world regexes, showing that they capture the wide majority of IA regexes (\cref{section:Experiment1}).
	\item A human-subjects evaluation of the usability of our proposed approach, showing that our approach gave developers greater understanding than existing approaches when detecting and repairing \REDOS regexes (\cref{sec:Experiment3}).
	%\item A second human-subjects evaluation, showing that our IA anti-patterns and fix patterns consistently provided higher understanding of what makes regexes vulnerable and what makes repaired regexes not vulnerable than when developers applied only existing tools (\cref{sec:Experiment3}).
\end{enumerate}
































% \begin{figure}[ht] 
%     \centering 
%     \begin{minipage}[b]{0.18\columnwidth}
%       \centering
%       \begin{tikzpicture}[baseline=-1.80em,initial text=]
%         %[initial text=]
%         \tikzstyle{every state}=[inner sep=0pt, minimum size=0.2cm]

%         \node[state, initial, initial distance=0.25cm]     (q1) {$$}; 
%         \node[state, right = 0.4cm of q1, accepting] (q2) {$$}; 
%         %\node[state, right of=q2, accepting] (q3) {$$}; 
%         \draw [->] (q1) edge node [above] {\tt $a$} (q2);
%         %\draw [->] (q2) edge node [above] {\tt $b$} (q3);
%       \end{tikzpicture} 
%       \caption*{\hspace{0.5cm}$a$}
%     \end{minipage} 
%     \begin{minipage}[b]{0.18\columnwidth}
%       \centering
%       \begin{tikzpicture}[baseline=-1.80em,initial text=]
%         \tikzstyle{every state}=[inner sep=0pt, minimum size=0.2cm]

%         \node[state, initial, initial distance=0.25cm]     (q1) {$$}; 
%         \node[state, above = 0.3cm of q1] (q2) {$$}; 
%         \node[state, right = 0.3cm of q1, accepting] (q3) {$$}; 
%         \draw [->] (q1) edge node [left] {\tt $a$} (q2);
%         \draw [->] (q2) edge node [above, pos=0.75] {\tt $b$} (q3);
%       \end{tikzpicture} 
%       \caption*{\hspace{0.5cm}$a \cdot b$}
%     \end{minipage} 
%     \begin{minipage}[b]{0.18\columnwidth}
%       \centering
%       \begin{tikzpicture}[baseline=-1.80em,initial text=]
%         \tikzstyle{every state}=[inner sep=0pt, minimum size=0.2cm]

%         \node[state, initial, initial distance=0.25cm]     (q1) {$$}; 
%         \draw (q1) edge[loop above] node [left] {\tt $a$} (q1);
%         \node[state, right = 0.4cm of q1, accepting] (q2) {$$}; 
%         \draw [->] (q1) edge node [above] {\tt $\epsilon$} (q2);
%       \end{tikzpicture} 
%       \caption*{\hspace{0.45cm}$a*$}
%     \end{minipage} 
%     \begin{minipage}[b]{0.18\columnwidth}
%       \centering
%       \begin{tikzpicture}[baseline=0em,initial text=]
%         \tikzstyle{every state}=[inner sep=0pt, minimum size=0.2cm]

%         \node[state, initial, initial distance=0.25cm]     (q1) {$$}; 
%         \node[state, above right = 0.4cm of q1]     (q2) {$$}; 
%         \node[state, below right = 0.4cm of q1]     (q3) {$$}; 
%         \node[state, below right = 0.4cm of q2, accepting]     (q4) {$$}; 
%         \draw [->] (q1) edge node [above, pos=0.25] {\tt $\epsilon$} (q2);
%         \draw [->] (q1) edge node [below, pos=0.25] {\tt $\epsilon$} (q3);
%         \draw [->] (q2) edge node [above, pos=0.75] {\tt $a$} (q4);
%         \draw [->] (q3) edge node [below, pos=0.75] {\tt $b$} (q4);
%       \end{tikzpicture} 
%       \caption*{\hspace{0.6cm}$a \vert b$}
%     \end{minipage} 
%     \hspace{0.02\columnwidth}
%     \vline
%     %\hspace{0.01\columnwidth}
%     \begin{minipage}[b]{0.18\columnwidth}
%       \centering
%       \tikzset{invisible/.style={minimum width=0mm,inner sep=0mm,outer sep=0mm}}
%       \begin{tikzpicture}%[baseline=(current bounding box.north)]
%         [initial text=]
%         \tikzstyle{every state}=[inner sep=0pt, minimum size=0.2cm]

%         % \node[state, initial]     (q1) {$$}; 
%         % \node[state, right of=q1, accepting] (q2) {$$}; 
%         % %\node[state, right of=q2, accepting] (q3) {$$}; 
%         % \draw [->] (q1) edge node [above] {\tt $a$} (q2);
%         % %\draw [->] (q2) edge node [above] {\tt $b$} (q3);

%         \node[state, initial, initial distance=0.25cm] (q1) {$$};
%         %\node[state, right = of q1] (q2) {$q_2$};
%         \node[state, above right = 0.4cm of q1] (q2) {$$};
%         \node[state, below right = 0.4cm of q1] (q3) {$$};
%         \node[state, below right = 0.4cm of q2, accepting] (q4) {$$};

%         \draw[->] (q1) edge [] node [above, pos=0.25] {\tt $\epsilon$} (q2);
%         \draw[->] (q1) edge [] node [below, pos=0.25] {\tt $\epsilon$} (q3);
%         \draw[->] (q2) edge [] node [above, pos=0.75] {\tt $a$} (q4);
%         \draw[->] (q3) edge [] node [below, pos=0.75] {\tt $a$} (q4);

%         \node[label=left:{$\epsilon$}, above= 0.47cm of q1,invisible] (above1) {};
%         \draw (q4) |- (above1);
%         \draw[->] (above1) -- (q1);
%       \end{tikzpicture} 
%       \caption*{\hspace{0.7cm}$(a \vert a)$+}
%     \end{minipage}
%     % \caption{
%     %     \KREsAcro operators and NFA equivalents for character, concatenation, repetition, and disjunction.
%     %     NFAs for \KREsAcros have in-degree and out-degree $\leq 2$, although this is higher under $\epsilon$-closure.
%     %     The final figure shows an exponentially ambiguous \KREsAcro.
%     % }
%     \label{figure:regex2NFA} 
% \end{figure} 

% \begin{table}
%     % DECREASE FONT SIZE?
%     %\scriptsize
%     %\footnotesize
%     %\small
%     \centering
%     \caption{
%       Regexes, time complexity, and the length of problematic input $|w|$ that necessitates a 10-second regex match in \TODO{Java-OpenJDK-X.XX}.
%       Each of these exhibits slow behavior on the input ``a$\stackrel{n}{\cdots}$ab''.
%       Machine is desktop class (\TODO{CPU specs go here}).
%     }
%     \begin{tabular} {cccc}
%     \toprule
%     \textbf{Regex}  & \textbf{Complexity}   & \textbf{$|w|$} \\
%     \toprule
%     \verb<^a*a*$<   & $\mathcal{O}(|w|^2)$  & ? \\
%     \verb<^a*a*a*$< & $\mathcal{O}(|w|^3)$  & ? \\
%     \verb<^(a|a)*$< & $\mathcal{O}(2^{|w|})$ & ? \\
%     \verb<^(a*)*$<  & $\mathcal{O}(2^{|w|})$ & ? \\
%     \bottomrule
%     \label{table:RegexQueryResponseTiming}
%     \end{tabular}
%     \vspace{-0.30cm}
% \end{table} 



==> intro-new.tex <==
%!TEX root = main.tex

\DY{We may want to revisit the title later. Now I see some important keywords include: usability, understandability, regex modality, anti-pattern, and fix strategies.}
\JD{I agree. Since this is a second submission, perhaps we can put this request into the letter to the reviewers?}

%%%
% 30K view
%%%
Regular expressions (\emph{regexes}) are a common software engineering tool for text processing~\cite{Chapman2016RegexUsageInPythonApps,Davis2018EcosystemREDOS}.
Regexes are used across the system stack~\cite{Li2008REL,Gogte2016HARE,Chiticariu2011SystemT,efftinge2006oaw}, including in security tasks such as
input validation~\cite{Balzarotti2008Saner,Wassermann2008XSS}
and
web application firewalls~\cite{ModSecurityWAFRuleset,ClamAVRegexRules}.
Unfortunately, regexes can themselves cause a security vulnerability because of the high worst-case time complexity of backtracking-based regex engine implementations.
This algorithmic complexity vulnerability is known as 
\emph{Regular Expression Denial of Service (\REDOS)}~\cite{Crosby2003REDOS,Roichman2009ReDoS}.
For example, \REDOS caused service outages at Stack Overflow in 2016~\cite{2016StackOverflowOutage} and at Cloudflare in 2019~\cite{Cloudflare2019REDOSPostMortem}.
Researchers report hundreds of vulnerable regexes in the software supply chain~\cite{Davis2018EcosystemREDOS} and in live web services~\cite{Staicu2018REDOS,barlas2022REDOS}.

%%%
% Existing solutions, vision
%%%
Given the severity and prevalence of \REDOS, 
researchers have developed
% characterizations of vulnerable regexes, \eg~\cite{Weideman2016REDOSAmbiguity,Wustholz2017Rexploiter,Davis2018EcosystemREDOS}.
% Researchers have also proposed
automatic tools to
detect, \eg~\cite{Berglund2014REDOSTheory,Weideman2016REDOSAmbiguity,Weideman2017StaticExpressions,Wustholz2017Rexploiter,liu21sp,Kirrage2013rxxr,Rathnayake2014rxxr2,Sugiyama2014RegexLinearityAnalysis,Sulzmann2017DerivAmbig,Shen2018ReScueGeneticRegexChecker}, and
fix vulnerable regexes, \eg~\cite{VanDerMerwe2017EvilRegexesHarmless,codykenny17,li2020flashregex,claver2021regis}.
However, although these approaches were effective in automated experiments~\cite{Davis2018EcosystemREDOS,Davis2019RegexGeneralizability}, past work did not examine their \emph{usability} when applied by humans.
\FS{Double check this claim above.}
Low usability often leads to human errors, reducing tool effectiveness.
\FS{Citation needed}
It also leads to tool refusal, \eg 95\% of developers reject tools when they cannot understand the results~\cite{johnson2013don}. 
% Effectiveness, Efficiency, Satisfaction, and Learnability







%%%
% Our approach, vision
%%%
In this paper, we propose a collection of \emph{anti-patterns} and \emph{fix strategies} 
to improve the usability of existing tools to detect and fix vulnerable regexes.
Our approaches are used in combination with existing tools, and improve their usability by improving the understandability of the resulting detected or fixed regex.
Developers obtain high understanding when tools provide examples and support to avoid repeating problems \cite{johnson2013don}.
Our anti-patterns improve the result understanding of detection tools by serving as examples to understand what makes a regex vulnerable and to avoid composing them in the future.
Developers also obtain high understanding when tools provide proposed fixes \cite{johnson2013don}.
Our fix strategies improve the result understanding of fix tools by serving as additional proposed fixes.

%%%
% Our approach, technical
%%%
To create our anti-patterns and fix strategies, we first develop a novel theory of regex infinite ambiguity (IA).
The IA region of a regex is a necessary component of \REDOS.
It is also the region that developers fix when they fix vulnerable regexes~\cite{Davis2018EcosystemREDOS}.
\FS{Double check this claim above.}
From our theory, we derived our IA anti-patterns, and from them, we derived our IA fix strategies.

%%%
% Existing solutions, technical
%%%
Our IA anti-patterns differ from previous characterizations of vulnerable regexes, \eg NFA-based~\cite{Weideman2016REDOSAmbiguity,Wustholz2017Rexploiter}, because they are based on the modality of the regex language, which is what most developers better or only understand~\cite{bai2019exploring,wang2019exploring}.
The only other characterization of vulnerable regexes that was proposed in the regex modality was found to be highly imprecise~\cite{Davis2018EcosystemREDOS}.
Our IA fix strategies are the first systematic characterization of approaches to fix vulnerable regexes, to the extent of our knowledge.

%%%
% Evaluation
%%%
We evaluate our IA anti-patterns and IA fix strategies formulating multiple research questions.
% RQ1 and RQ2 evaluate our anti-patterns by themselves, and RQ3 and RQ4 evaluate our anti-patterns and fix strategies complementing existing tools.
\emph{(RQ1: Comprehensivenes of anti-patterns) Do our IA anti-patterns characterize IA effectively in a large variety of regexes?}
\emph{(RQ2: Usability of anti-patterns) Are our IA anti-patterns usable enough for developers to detect IA effectively in the absence of tools?}
\emph{(RQ3: Usability of detection tools) Do our IA anti-patterns improve the result understandability of automatic tools to detect vulnerable regexes?}
\emph{(RQ4: Usability of fix tools) Do our IA fix strategies improve result understandability when using automatic tools to fix vulnerable regexes?}
To the extent of our knowledge, this is the first study to evaluate the usability of characterizations or tools to identify or fix vulnerable regexes.
\FS{Does this list of research questions follow naturally from the narrative before it? I think RQ3 and RQ4 are well motivated, but RQ1 and RQ2 may be less so. This is somewhat intentional, since I want RQ3 and RQ4 to be the key part of this work. But I don't want to confuse the reader too much. Thoughts?}


% In our evaluation, our anti-patterns achieved these goals.
Our evaluation provided multiple findings.
For RQ1, we proved the soundness and completeness of our underlying theory of regex infinite ambiguity (\cref{section:Theory,section:Appendix-Proofs}).
We also further validated the proof with an experiment and found that our anti-patterns provided much higher effectiveness (100\% precision, 99\% recall) than existing anti-patterns in the regex modality~\cite{Davis2018EcosystemREDOS} (50\% precision, 87\% recall) when applied over a large-scale dataset of \AnalyzedNRegexes real-world regexes \cite{Davis2019LinguaFranca} (\cref{section:Experiment1}).
For RQ2, we found that even beginner and intermediate developers (100\% of \HumanSubjectsN studied) effectively identified IA in regexes, in 5 different regex tasks, greatly improving over existing anti-patterns (50\%).
For RQ3, we found that open-source developers (\TODO{X\%} of \TODO{Y} studied) consistently improved their understanding of what makes the detected regex vulnerable when they complemented the detection tool with our anti-patterns.
 % of the results of a detection tool when they used our anti-patterns in combination with it.
They also consistently (\TODO{Z\%}) reported that they found them helpful and would continue using them in the future.
\FS{I'm not saying anything about RQ3 being more realistic than RQ2. Do we want to emphasize that aspect here?}
For RQ4, we found that open-source developers (\TODO{A\%} of \TODO{Y} studied) also consistently improved their understanding the resulting fixed regex when they complemented the fix tool with our fix strategies.
They also consistently (\TODO{B\%}) found our fix strategies helpful and plan to continue using them in the future.


% contributions
% \FS{TODO: These contributions need to be revisited, but everything above is done.}
% In summary, t
This paper provides the following contributions:
\begin{enumerate}
  \item A sound, complete theory of regex infinite ambiguity (IA) (\cref{section:Theory}).
  \item IA Anti-patterns (\cref{section:AntiPatterns}), derived from our theory, and IA fix strategies (\cref{sec:fix_strategies}), derived from them.
  \item A quantitative evaluation of the comprehensiveness of our IA anti-patterns over a large-scale of real-world regexes, showing that they capture IA effectively in the wide majority of them (\cref{section:Experiment1}).
  \item The first usability evaluation of characterizations of vulnerable regexes, showing that our IA anti-patterns were usable enough for novice developers to apply effectively in the absence of tools (\cref{sec:Experiment2}).
  \item The first usability evaluation of tools to detect and fix vulnerable regexes, showing that our IA anti-patterns and IA fix strategies improved their usability by improving their understanding (\cref{sec:Experiment3}).
  % characterizations of vulnerable regexes, showing that our IA anti-patterns were usable enough for novice developers to apply effectively in the absence of tools.
  % \item A human-subjects evaluation of the usability of our proposed approach, showing that our approach gave developers greater understanding than existing approaches when detecting and repairing \REDOS regexes (\cref{sec:Experiment3}).
  %\item A second human-subjects evaluation, showing that our IA anti-patterns and fix patterns consistently provided higher understanding of what makes regexes vulnerable and what makes repaired regexes not vulnerable than when developers applied only existing tools (\cref{sec:Experiment3}).
\end{enumerate}




























==> intro-new2.tex <==
%!TEX root = main.tex

\DY{We may want to revisit the title later. Now I see some important keywords include: usability, understandability, regex modality, anti-pattern, and fix strategies.}
\JD{I agree. Since this is a second submission, perhaps we can put this request into the letter to the reviewers?}
\JD{On consideration, let's just change the title here and discuss in the letter}

%%%
% 30K view
%%%
Regular expressions (\emph{regexes}) are a common software engineering tool for text processing~\cite{Chapman2016RegexUsageInPythonApps,Davis2018EcosystemREDOS}.
Regexes are used across the system stack~\cite{Li2008REL,Gogte2016HARE,Chiticariu2011SystemT,efftinge2006oaw}, including in security tasks such as
input validation~\cite{Balzarotti2008Saner,Wassermann2008XSS}
and
web application firewalls~\cite{ModSecurityWAFRuleset,ClamAVRegexRules}.
Unfortunately, regexes can themselves cause a security vulnerability because of the high worst-case time complexity of backtracking-based regex engine implementations.
This algorithmic complexity vulnerability is known as 
\emph{Regular Expression Denial of Service (\REDOS)}~\cite{Crosby2003REDOS,Roichman2009ReDoS}.
For example, \REDOS caused service outages at Stack Overflow in 2016~\cite{2016StackOverflowOutage} and at Cloudflare in 2019~\cite{Cloudflare2019REDOSPostMortem}.
Researchers report hundreds of vulnerable regexes in the software supply chain~\cite{Davis2018EcosystemREDOS} and in live web services~\cite{Staicu2018REDOS,barlas2022REDOS}.

%%%
% Existing solutions
%%%
\FS{I'm being intentionally verbose here, to pinpoint the 4 gaps filled by RQ1, RQ2, RQ3, and RQ4}
\DY{I understand the intention. But I felt that the second and third points can be merged to reduce redundancy.  I see that the first point is related to RQ1-3 and the second/third points are linked to RQ4-5. Nonetheless, I am fine with the current draft if you think verbosity helps here.}
\JD{I find the verbosity confusing. I've shortened the next paragraph, PTAL.}
%\FS{Please, double check all the claims in these paragraphs about related work.}
Many approaches have been proposed to address the \REDOS problem.
Our work builds on those that try to detect and repair regexes.
%Given the severity and prevalence of regexes vulnerable to \REDOS,  multiple approaches have been proposed to address them.
In this vein, some researchers taxonomized vulnerable regexes~\cite{Davis2018EcosystemREDOS} for manual use by developers.
%Manual approaches can be useful when tools disrupt developer workflow~\cite{johnson2013don}, \eg during regex composition or when working with simple regexes.
%Unfortunately, their automated experiment showed that this characterization is highly \emph{imprecise}~\cite{Davis2018EcosystemREDOS}.
Others proposed tools to automatically
  detect (~\cite{Berglund2014REDOSTheory,Weideman2016REDOSAmbiguity,Weideman2017StaticExpressions,Wustholz2017Rexploiter,liu21sp,Kirrage2013rxxr,Rathnayake2014rxxr2,Sugiyama2014RegexLinearityAnalysis,Sulzmann2017DerivAmbig,Shen2018ReScueGeneticRegexChecker})
  or repair (~\cite{VanDerMerwe2017EvilRegexesHarmless,codykenny17,li2020flashregex,claver2021regis})
  vulnerable regexes
All of these approaches have been evaluated solely via automated experiments. %, \eg~\cite{Davis2018EcosystemREDOS,Davis2019RegexGeneralizability}.
Their \emph{usability} by developers has not been studied, jeopardizing their impact in practice~\cite{johnson2013don}.
%Low usability often leads to lowered effectiveness, due to human errors,
%\FS{Citation needed}
%and even to complete tool refusal.
%For example, \eg 95\% of developers reject tools when they cannot understand the results~\cite{johnson2013don}. 

%%%
% Our vision
%%%
The goal of this paper is to complement these existing \REDOS approaches by improving their usability.
% Dimensions of usability: Effectiveness, Efficiency, Satisfaction, and Learnability
We focus on two dimensions of usability: the \emph{effectiveness} with which developers perform the detection or repair task, and their \emph{understanding} of the outcome.
\FS{Citation needed for dimensions of usability}
\FS{Add a sentence saying that our insight is that characterizations can improve the usability of automatic tools. We develop a novel characterization that is highly effective and we evaluate how much it improves usability.}



%%%
% Our vision, specific goals connected to earlier gaps
%%%
We aim to improve the \emph{effectiveness} of the existing characterization of vulnerable regexes~\cite{Davis2018EcosystemREDOS} by replacing it with a novel collection of \emph{anti-patterns}.
Our anti-patterns characterize a fundamental component of \REDOS: the infinitely ambiguous (IA) region of a vulnerable regex.
This is the region that the existing characterization characterizes~\cite{Davis2018EcosystemREDOS}, that many detection tools detect, \eg~\cite{Weideman2016REDOSAmbiguity,Wustholz2017Rexploiter}, and that developers often repair in vulnerable regexes~\cite{Davis2018EcosystemREDOS}.
To provide high effectiveness, we ground our anti-patterns in a novel theory of regex infinite ambiguity (IA), which we also developed.

We aim to improve the \emph{understanding} of the outcome of automatic detection tools~\cite{Berglund2014REDOSTheory,Weideman2016REDOSAmbiguity,Weideman2017StaticExpressions,Wustholz2017Rexploiter,liu21sp,Kirrage2013rxxr,Rathnayake2014rxxr2,Sugiyama2014RegexLinearityAnalysis,Sulzmann2017DerivAmbig,Shen2018ReScueGeneticRegexChecker} by complementing them with our \emph{anti-patterns}.
Developers improve their understanding when tools provide: 
examples and
support to avoid repeating problems
\cite{johnson2013don}.
We expect that our \emph{anti-patterns} will complement detection tools serving as examples to understand what makes a vulnerable regex and 
to avoid composing them in the future.

We aim to improve the \emph{understanding} of the outcome of automatic repair tools~\cite{VanDerMerwe2017EvilRegexesHarmless,codykenny17,li2020flashregex,claver2021regis} by complementing them with a novel collection of \emph{fix strategies}.
We derived our fix strategies from our anti-patterns.
Developers also improve their understanding when tools provide
proposed repairs~\cite{johnson2013don}.
We expect that our \emph{fix strategies} will complement automatic repair tools tools serving as  proposed fixes that are easy to understand.

%%%
% Evaluation
%%%
We evaluated how much our anti-patterns and fix strategies achieve these goals.
First, we evaluated the improvement in \emph{effectiveness} provided by our anti-patterns over existing characterizations in multiple ways: (RQ1) we developed a proof for our theory of IA, 
\DY{First mention of IA in the intro. Should we define?}
(RQ2) we measured the effectiveness of our anti-patterns in an automatic experiment over a large dataset of regexes, and (RQ3) we measured their effectiveness when applied manually by humans in a scenario in which they would not use tools to not disrupt their workflow~\cite{johnson2013don}.
Then, (RQ4) we evaluated the improvement in \emph{understanding} provided by our anti-patterns when complementing existing detection tools.
Finally, (RQ5) we evaluated the improvement in \emph{understanding} provided by our fix strategies when complementing existing fixing tools.
\DY{Do we need the following bullet points here? They seem repetitive.}
Thus, our evaluation answered the following research questions:
\begin{itemize}
  \item \textbf{RQ1: Is our theory of IA sound and complete?}
  \item \textbf{RQ2: How effectively do our IA anti-patterns characterize IA in a large collection of regexes?}
  \item \textbf{RQ3: How effectively can humans apply our IA anti-patterns in the absence of tools?}
  \item \textbf{RQ4: How much do our IA anti-patterns improve the understanding of the outcome of  tools to detect vulnerable regexes?}
  \item \textbf{RQ5: How much do our IA fix strategies improve the understanding of the outcome of  tools to fix vulnerable regexes?}
\end{itemize}
To the extent of our knowledge, this is the first study to evaluate the usability of characterizations or tools to identify or fix vulnerable regexes.


%%%
% Results
%%%
% In our evaluation, our anti-patterns achieved these goals.
Our evaluation provided multiple findings.
For RQ1, we proved the soundness and completeness of our underlying theory of regex infinite ambiguity (\cref{section:Theory,section:Appendix-Proofs}).
For RQ2, we further validated the proof with an experiment and found that our anti-patterns provided much higher effectiveness (100\% precision, 99\% recall) than existing anti-patterns in the regex modality~\cite{Davis2018EcosystemREDOS} (50\% precision, 87\% recall) when applied over a large-scale dataset of \AnalyzedNRegexes real-world regexes \cite{Davis2019LinguaFranca} (\cref{section:Experiment1}).
For RQ3, we found that even beginner and intermediate developers (100\% of \HumanSubjectsN studied) effectively identified IA in regexes, in 5 different regex tasks, greatly improving over existing anti-patterns (50\%).
For RQ4, we found that open-source developers (\TODO{X\%} of \TODO{Y} studied) consistently improved their understanding of what makes the detected regex vulnerable when they complemented the detection tool with our anti-patterns.
 % of the results of a detection tool when they used our anti-patterns in combination with it.
They also consistently (\TODO{Z\%}) reported that they found them helpful and would continue using them in the future.
\FS{I'm not saying anything about RQ3 being more realistic than RQ2. Do we want to emphasize that aspect here?}
\DY{I don't see one is more realistic than the other.}
For RQ5, we found that open-source developers (\TODO{A\%} of \TODO{Y} studied) also consistently improved their understanding the resulting fixed regex when they complemented the fix tool with our fix strategies.
They also consistently (\TODO{B\%}) found our fix strategies helpful and plan to continue using them in the future.


% contributions
% \FS{TODO: These contributions need to be revisited, but everything above is done.}
% In summary, t
This paper provides the following contributions:
\begin{enumerate}
  \item A sound, complete theory of regex infinite ambiguity (IA) (\cref{section:Theory}).
  \item IA Anti-patterns (\cref{section:AntiPatterns}), derived from our theory, and IA fix strategies (\cref{sec:fix_strategies}), derived from them.
  \item A quantitative evaluation of the comprehensiveness of our IA anti-patterns over a large-scale of real-world regexes, showing that they capture IA effectively in the wide majority of them (\cref{section:Experiment1}).
  \item The first usability evaluation of characterizations of vulnerable regexes, showing that our IA anti-patterns were usable enough for novice developers to apply effectively in the absence of tools (\cref{sec:Experiment2}).
  \item The first usability evaluation of tools to detect and fix vulnerable regexes, showing that our IA anti-patterns and IA fix strategies improved their usability by improving their understanding (\cref{sec:Experiment3}).
  % characterizations of vulnerable regexes, showing that our IA anti-patterns were usable enough for novice developers to apply effectively in the absence of tools.
  % \item A human-subjects evaluation of the usability of our proposed approach, showing that our approach gave developers greater understanding than existing approaches when detecting and repairing \REDOS regexes (\cref{sec:Experiment3}).
  %\item A second human-subjects evaluation, showing that our IA anti-patterns and fix patterns consistently provided higher understanding of what makes regexes vulnerable and what makes repaired regexes not vulnerable than when developers applied only existing tools (\cref{sec:Experiment3}).
\end{enumerate}

\JD{This paper has many sections. I felt that some sign-posting here will help.}
This paper proceeds as follows.
\cref{section:Background} and~\cref{section:RelatedWork} present the background and related work.
In~\cref{section:Theory} we present our theory of regex infinite ambiguity.
From this theory, we
  derive anti-patterns (\cref{section:AntiPatterns})
  and
  fix strategies (\cref{sec:fix_strategies}).
We evaluate these contributions through
  automated analysis of a regex corpus (\cref{section:Experiment1:dataset}),
  a controlled experiment (\cref{sec:Experiment2}),
  and an in-the-wild experiment repairing zero-day \REDOS vulnerabilities (\cref{sec:Experiment3}).

==> intro-old.tex <==
%!TEX root = main.tex

\FS{@Dongyoon, @Jamie, can you please provide suggestions to shorten Sections 1, 2, 3 and 4?}
\JD{Shortening suggestion: The introduction is pretty wide-ranging. Let's focus it down to the typical 4+1-paragraph format: 30K view, related work, our approach, evaluation and results, contribution bullets.}

% background
Regular expressions (\emph{regexes}) are an important software engineering tool.
They are used in an estimated 30--40\% of open-source projects~\cite{Chapman2016RegexUsageInPythonApps,Davis2018EcosystemREDOS}.
Regexes use spans the system stack,
including for security-specific tasks
  (\eg input validation~\cite{Balzarotti2008Saner,Wassermann2008XSS},
   web application firewalls~\cite{ModSecurityWAFRuleset},
   and
   anti-virus~\cite{ClamAVRegexRules});
and for general-purpose tasks
  (\eg text processing~\cite{Li2008REL,Gogte2016HARE}
   and
   syntax highlighting~\cite{Chiticariu2011SystemT,efftinge2006oaw}).

% problem
Regexes may introduce a security vulnerability: \emph{Regular Expression Denial of Service (\REDOS)}~\cite{Crosby2003REDOS,Roichman2009ReDoS}.
\REDOS is an algorithmic complexity vulnerability~\cite{Crosby2003AlgorithmicComplexityAttacks}, denying service by exhausting computational resources.
In a \REDOS exploit, a regex's super-linear worst-case execution time is triggered during regex matching.
\REDOS can affect software that uses an unsafe (\emph{backtracking}) regex engine to evaluate a problematic (\emph{super-linear}) regex on untrusted strings (such as user input).
% wide impact:
Unsafe regex engines are common in practice, including the regex engines shipped in many popular programming languages, \eg Java, JavaScript, Ruby, and Python~\cite{Cox2007RegExBible,Davis2019LinguaFranca}. 
% serious problem
%Unsafe regex engines use a naive backtracking-based predictive parser, which 
This hazardous infrastructure exposes many web services to \REDOS. %, \eg to manipulate untrusted client data.
For example, \REDOS caused service outages at Stack Overflow in 2016~\cite{2016StackOverflowOutage} and at Cloudflare in 2019~\cite{Cloudflare2019REDOSPostMortem}.
Beyond those cases,
Davis \etal showed that the software supply chain has many vulnerable regexes~\cite{Davis2018EcosystemREDOS},
and
Staicu \& Pradel found that those regexes render hundreds of popular websites vulnerable to \REDOS~\cite{Staicu2018REDOS}.

% \begin{figure}[] 
%   \centering
%     \includegraphics[width=.95\linewidth]{figures/illustrations/swisscheese.pdf}
%     %\vspace{-5px}
%     \captionof{figure}{
%         The Swiss cheese model~\cite{reason1990contribution,reason2000human} (defense in depth) for \REDOS. 
%         Most existing techniques to address \REDOS-vulnerable regexes are applied during their maintenance or after their deployment.
%         Our work provides early prevention, avoiding the composition of vulnerable regexes in the first place.
%         %avoiding composition of vulnerable regex
%         %(
%         %theory and anti-patterns
%         %),
%         %coping with vulnerable regexes
%         %(
%         %detecting SL regexes,
%         %repairing SL regexes,
%         %recovering from REDOS 
%         %),
%         %changing the infrastructure 
%         %(
%         %changing the regex engine
%         %)
%         %}
%         % \DY{Figure updated.}
%     }
%     \label{fig:swisscheese}
% \end{figure}




% \iffalse
% \begin{table}[]
% \begin{tabular}{p{2.6cm}|p{2.55cm}|p{2.55cm}}
% \hline
% \textbf{Existing Techniques for the Composition Stage}     & \textbf{Existing Techniques for the Maintenance Stage}          & \textbf{Existing Techniques for the Deployment Stage}                          \\
% \hline
% \hline
% Unsound anti-patterns~\cite{Davis2018EcosystemREDOS} & Detection techniques~\cite{Berglund2014REDOSTheory,Weideman2016REDOSAmbiguity,Weideman2017StaticExpressions,Wustholz2017Rexploiter,liu21sp,Kirrage2013rxxr,Rathnayake2014rxxr2,Sugiyama2014RegexLinearityAnalysis,Sulzmann2017DerivAmbig,Shen2018ReScueGeneticRegexChecker} & Infrastructure defense techniques~\cite{Cox2010RE2Implementation,davis2021using,bai2021runtime}  \\
% \hline
% \textbf{This work}: sound and complete theory, and derived anti-patterns          & Repair techniques~\cite{VanDerMerwe2017EvilRegexesHarmless,codykenny17,li2020flashregex,claver2021regis}    &                                    \\
% \end{tabular}
% \caption{Most existing techniques to address \REDOS-vulnerable regexes are applied during their maintenance or after their deployment. 
% Our work provides early prevention, avoiding the composition of vulnerable regexes in the first place.}
% % \vspace{-.1in}
% \label{tab:existingWork}
% \end{table}


% \begin{table}[]
% \begin{tabular}{@{}lp{7cm}@{}}
% \toprule
% Stage       & Techniques \\ \hline
% Maintenance & Detection techniques~\cite{Berglund2014REDOSTheory,Weideman2016REDOSAmbiguity,Weideman2017StaticExpressions,Wustholz2017Rexploiter,liu21sp,Kirrage2013rxxr,Rathnayake2014rxxr2,Sugiyama2014RegexLinearityAnalysis,Sulzmann2017DerivAmbig,Shen2018ReScueGeneticRegexChecker} \\ \hline
%             & Repair techniques~\cite{VanDerMerwe2017EvilRegexesHarmless,codykenny17,li2020flashregex,claver2021regis} \\ \hline
% Deployment  & Infrastructure defense~\cite{VanDerMerwe2017EvilRegexesHarmless,codykenny17,li2020flashregex,claver2021regis} \\ \hline
% Composition & Unsound anti-patterns~\cite{Davis2018EcosystemREDOS} \\ \hline
% (This work) & sound and complete theory, and derived anti-patterns \\ \hline
% \end{tabular}
% \end{table}
% \fi


% existing solutions (other layers)
Given the severity and prevalence of \REDOS, researchers have proposed mechanisms to defend against it.
%(see Table~\ref{tab:existingWork}).
The majority of them proposed tools to automatically
% apply to the software maintenance stage ---to 
% focus on automatically 
identify~\cite{Berglund2014REDOSTheory,Weideman2016REDOSAmbiguity,Weideman2017StaticExpressions,Wustholz2017Rexploiter,liu21sp,Kirrage2013rxxr,Rathnayake2014rxxr2,Sugiyama2014RegexLinearityAnalysis,Sulzmann2017DerivAmbig,Shen2018ReScueGeneticRegexChecker} or repair~\cite{VanDerMerwe2017EvilRegexesHarmless,codykenny17,li2020flashregex,claver2021regis} vulnerable regexes.
% --- or after software deployment~\cite{Cox2010RE2Implementation,davis2021using,bai2021runtime}.

{\color{blue}
% limitations of existing work
However, developers often choose to not use automated tools that are available to them, due to various barriers \cite{johnson2013don}.
The most common and definite barrier limiting adoption of automated tools (reported by 95\% of studied developers) is result understandability \cite{johnson2013don}.
Developers become discouraged from using an automated tool when they cannot clearly understand its output.
% \emph{``Nineteen of our 20 participants, felt that many static analysis tools do not present their results in a way that gives enough information for them to assess what the problem is, why it is a problem and what they should be doing differently.''}

In this paper, we propose novel approaches to support developers to (1) identify and (2) repair vulnerable regexes that provide higher result understandability than existing approaches based on automated tools.
They particularly improve the understanding of
% to (1) identify and (2) fix vulnerable regexes that provide higher understanding 
% ---particularly of 
(1) what makes a regex vulnerable and (2) what makes a repaired regex not vulnerable any more.
Our approach is based on (1) anti-patterns that characterize regexes that are vulnerable to \REDOS and (2) fix patterns that propose strategies to repair them.
We developed a novel theory of regex infinite ambiguity (IA) ---a necessary component of \REDOS.
Then, we derived our collections of (1) IA anti-patterns and (2) IA fix-patterns from it.
We thus leverage our foundational contribution to enable practical ones.
% We finally complement our IA anti-patterns with a collection of fix patterns to support developers in repairing their vulnerable regexes.
% Developers also report that proposed fixes improve tool understanding and usage \cite{johnson2013don}).

\FS{Is it ok to be a bit speculative in this paragraph below?}
\DY{I think it is okay. I suggest we add some discussion about why/how ours improve understandability. We already talk about ``examples''. Besides, I thought it is worth/safe to emphasize regex-level modality.}
Our proposed IA anti-patterns and fix-patterns complement existing automated tools to identify and fix regexes vulnerable to \REDOS.
We expect developers to use both approaches in combination.
Automated tools allow the detection of vulnerable regexes efficiently in large codebases.
Our anti-patterns and fix-patterns allow developers to assess and repair them with high understanding.
Common aspects that developers require to improve their understanding of tool results are: examples, support to avoid repeating problems, and proposed fixes \cite{johnson2013don}.
Developers can use our IA anti-patterns as examples to identify existing vulnerable regexes and to avoid composing vulnerable regexes in the future.
They can apply our IA anti-patterns at regex composition time, allowing them to repair their regexes even before they are introduced in the codebase.
Developers can also use our IA fix-patterns as proposed fixes to repair their vulnerable regexes.
\FS{Is it useful to also mention developer education in secure coding as a benefit?}


% \FS{Is this final sentence useful?}
% Furthermore, our IA anti-patterns and fix patterns can be applied early, as regexes are being composed, allowing developers to fix vulnerable regexes even before they are introduced in their codebases.
% Since our anti-patterns are applied by developers in their heads, they have additional benefits: they educate developers in secure coding~\cite{gasiba21}, and they are easily applied early, during regex composition, when the regex is easier to fix.
% An additional benefit of our anti-patterns is that they can be applied in developer's minds at composition time, identifying vulnerable regexes early, \ie as they are being composed, making them easier to fix.
% Our anti-patterns also deducate developers in secure coding ---a valuable complement to automated security tools~\cite{gasiba21}.


% Developers can use them as examples to identify what regexes are vulnerable and to avoid composing vulnerable regexes in the future.
% \FS{Is this claim of avoiding future composition of vulnerable regexes unsupported by our data, or is it ok to speculate a little here?}
% Developers report that examples and support to avoid repeating problems improve their understanding of technique results \cite{johnson2013don}.

% Developers also report that proposed fixes improve tool understanding and usage \cite{johnson2013don}).














% % our idea: the gist
% % \JD{Too many hyphens. Feels like headlines instead of complete sentences.}
% In this paper, we set a different goal: \textbf{preventing the introduction of \REDOS in the first place} ---at regex composition time, as illustrated in~\cref{fig:swisscheese}.
% We propose a novel theory of regex infinite ambiguity (IA) ---a necessary component of \REDOS--- and derive a collection of anti-patterns from it.
% We thus leverage our foundational contribution to enable a practical one.
% Developers can apply our anti-patterns at composition time to avoid introducing infinitely ambiguous (IA) regexes in their source code, and thus avoid \REDOS.


% % why many layers
% % Our proposed work fills a gap in the layers of defense against \REDOS, providing a coding standard to prevent it at composition time.
% %\FS{It's weird to mention a gap here, since there is no gap in Table~\ref{tab:existingWork}.}
% %\DY{I agreed on the current tone/claim.}
% Our proposed theory and anti-patterns fill a gap in the existing multi-layer defense against \REDOS, providing a coding standard to prevent it at composition time instead of at maintenance or deployment time.
% %The existing approaches target the software maintenance and deployment stages, and we propose a novel approach to target the regex composition stage.
% Our approach aligns with the multi-layer approach to software security known as \emph{defense in depth} \cite{stytz2004considering}, or the \emph{Swiss cheese} approach \cite{kamoun2014human,reason1990contribution,reason2000human}.
% When using many layers to defend against security problems, the strengths of each layer can counterbalance the limitations of the others.
% Also, different defense layers may better fit the workflow of different software development teams.
% \FS{@FS: Refine argument. It's not only about composition. It's also about complementing existing tools for understandability.}
% % \FS{Argument: any anti-pattern improves usability over existing tools. Experiments 1 measures which anti-patterns are best: Davis or ours. Experiment 2 measures whether usability is actually better when using anti-patterns.}






% what else could one use?
%   our contributions on top of it
% \JD{Move this content earlier, to go just after the swiss cheese paragraph?}
% To the extent of our knowledge, only two existing approaches may (partially) support developers to avoid composing IA regexes, both of which are limited.
To the extent of our knowledge, only one existing theory and one set of anti-patterns currently (partially) characterize regexes vulnerable to \REDOS.
}
First, Brabrand \& Thomsen's theory~\cite{brabrand2010typed} characterizes ambiguous regexes, but does not distinguish between finite (safe) and infinite (unsafe) ambiguity.
Our proposed theory improves upon Brabrand \& Thomsen's by soundly and completely characterizing infinitely ambiguous regexes.
% \DY{The following sentence does not seem complete.}
Second, existing 
% \JD{anti patterns gobefore brabrand sentebce}  
anti-patterns in reference texts characterize regexes vulnerable to \REDOS~\cite{Friedl2002MasteringRegexes,Goyvaerts2006CompleteTutorial,safeRegexHomePage,Goyvaerts2012Cookbook}.
% \JD{Instead of ``state-of-the-practice (SOP)'', can we just refer to ``existing anti-patterns''?}
However, a recent study found that they are insufficient ---they have a large ratio of false positives~\cite{Davis2018EcosystemREDOS}.
Our proposed IA anti-patterns improve upon existing anti-patterns by being derived from a formal theory of infinite ambiguity, and achieving high precision and recall as a result.

% % why an early layer (composition time)
% As a prevention measure, our proposed work also follows the growing trend in software security of \emph{shifting left} security concerns ---addressing them early in the life-cycle to achieve benefits in cost savings, quality control, and speed to market \eg \cite{shiftleft1,shiftleft2,shiftleft3}.
% More generally, in software engineering, it is common wisdom that problems detected earlier are easier and cheaper to fix ---driving common practices like continuous integration~\cite{hilton2016usage} and modern code review~\cite{bacchelli2013expectations}.
% Also, since we designed our anti-patterns for developer comprehension, we contribute to the important mission of educating software developers in secure coding ---as a valuable complement to automated security tools~\cite{gasiba21}.
% % \JD{Can we point to any other examples of collections of security patterns/anti-patterns?. It would be nice to join an existing conversation about patterns instead of trying to invent one. For example, there are a bunch of security patterns (divided into Arch/Design/Implementation-level) in \url{https://apps.dtic.mil/sti/citations/ADA636498}. I think our regex anti-patterns are an example of an implementation-level (anti-)pattern. Indeed Davis \etal~\cite{Davis2018EcosystemREDOS} motivates anti-patterns and points to existing anti-patterns from practitioner texts, but it is easy for us to show the shortcomings of that approach --- Davis's data points to inaccuracies that we think we can improve on.}


% \JD{combien the first two eval paragraphs? both involve theory+formulation, and then the second eval paragraph covers human-subjects experient}
% evaluation
%   we improve (and evaluate) brabrand with the theory (and proofs), and we improve davis with the anti-patterns (and the 2 experiments).
% \JD{Starting in this paragraph and perhaps the next one too, add forward references to the relevant sections.}
% \JD{flip this sentence so we reference theory and then point to appendix.}
We evaluated our proposed approaches.
For our IA regex theory (\cref{section:Theory}), we proved (\cref{section:Appendix-Proofs}) its soundness and completeness.
To evaluate our anti-patterns (\cref{section:AntiPatterns}), we performed three complementary experiments (\cref{section:Experiment1}, \cref{sec:Experiment2}, and \cref{sec:Experiment3}).
First, we evaluated the effectiveness of our anti-patterns for comprehensiveness (\cref{section:Experiment1}) by applying them to a large-scale dataset of
 % \AnalyzedNRegexes 
real-world regexes~\cite{Davis2019LinguaFranca}
% \JD{The size of the dataset is not particularly interesting here, unless we're both (a) trying to do a head-to-head comparison on \REDOS-detection techniques; and (b) showing the dataset is better. Since we are not, I don't think we should mention the size here at all. I think it's OK to mention it deep in the evaluation section, like we currently do later on.}
% --- one order of magnitude larger than the evaluations performed for \REDOS-detection techniques for other development stages, \eg \cite{liu21sp,Shen2018ReScueGeneticRegexChecker,Weideman2016REDOSAmbiguity,Weideman2017StaticExpressions}.
Our experiments showed that our anti-patterns provide higher precision and recall than existing anti-patterns ---100\% vs. 50\% precision, and 99\% vs. 87\% recall.
We also learned that two of our six anti-patterns (Concat 1 and Concat 2) are enough to cover a wide majority of IA regexes (99\%) in practice.
{\color{blue}
Second, we evaluated our anti-patterns in a preliminary human-subjects study, in which developers applied them during regex composition (\cref{sec:Experiment2}).
This second experiment ($N=\HumanSubjectsN$) showed that all our studied practitioners (100\%) successfully identified whether their composed regex was IA for all our 5 studied tasks, greatly improving over existing anti-patterns (50\%).
This experiment also showed that our IA anti-patterns only helped X\% of developers to fix their composed regex when it was IA.
\FS{Fill in that X\%}
Therefore, we also developed a collection of fix patterns, to support developers to repair their composed regexes when they identify them as IA.
Third, we performed a final human-subjects study to assess the extent to which our IA anti-patterns and fix patterns complement existing tools for the same goals by providing higher understanding.
This study showed that \dots
\FS{TODO: Fill in after analysis.}
}

% Second, we also evaluated the usability of our anti-patterns at regex composition time (\cref{sec:Experiment2}).
% Our human-subjects experiment ($N=\HumanSubjectsN$) showed that all our studied practitioners (100\%) successfully applied our anti-patterns during regex composition for all our 5 studied tasks, greatly improving the success that they achieved when applying existing anti-patterns (50\%).



%\JD{@Adnan please replace all numbers with macros defined in the data/data.tex file.}
%\AH{@Jamie, Sorry I did not find the macros. The file looks empty to me.}
%\JD{You are supposed to populate it with your data macros, so that you don't make typos when you use the number in several places in the paper.}


% We evaluated our contributions through proofs and experiments.
% We evaluated our regex IA theory using proofs to reason about its soundness and completeness.
% Then, we evaluated our regex IA anti-patterns in two complementary ways, to understand their benefits in breadth and in depth.
% In breadth, we measured their effectiveness to capture IA over a large, diverse collection of real-world regexes.
% In depth, we studied how they helped developers avoid composing IA regexes in practice, in a human subjects experiment.
% Our evaluation answers the following research questions:

% \FS{
%   Add a list of contributions:

%   - We are the first to conduct experiments on the efficacy of regex-based anti-patterns, with anti-patterns grounded in our novel analysis of regex ambiguity rather than after a conversion to automata.
% }
% \JD{Something we've discussed in meetings: Our ability to measure the value of the anti-patterns is distinctive...Should other people do this approach in other contexts? Contrast with qualitative research methods that yield anti-patterns?}
% \FS{I agree, but I can't think of a good sentence to argue that, because making a claim about anti-patterns in general would cover too much literature.}

% contributions
This paper provides the following contributions:
\begin{enumerate}
  \item A novel theory that soundly and completely characterizes regex infinite ambiguity (\cref{section:Theory}).
  \item A collection of (IA) anti-patterns of regex infinite ambiguity, derived from our theory, to apply at composition time to avoid inserting regexes vulnerable to \REDOS (\cref{section:AntiPatterns}).
  \item An evaluation of the comprehensiveness of our proposed IA anti-patterns over a large-scale of real-world regexes, showing that they could capture the wide majority of IA regexes (\cref{section:Experiment1}).
{\color{blue}
  \item A human-subjects evaluation, showing that developers could effectively apply our IA anti-patterns to identify if their composed regexes were IA, and that some developers could also fix them when they were. (\cref{sec:Experiment2}).
  \item A collection of fix patterns to repair IA regexes (\cref{section:FixPatterns}).
  \item A second human-subjects evaluation, showing that our IA anti-patterns and fix patterns consistently provided higher understanding of what makes regexes vulnerable and what makes repaired regexes not vulnerable than when developers applied only existing tools (\cref{sec:Experiment3}).
}
\end{enumerate}
































% \begin{figure}[ht] 
%     \centering 
%     \begin{minipage}[b]{0.18\columnwidth}
%       \centering
%       \begin{tikzpicture}[baseline=-1.80em,initial text=]
%         %[initial text=]
%         \tikzstyle{every state}=[inner sep=0pt, minimum size=0.2cm]

%         \node[state, initial, initial distance=0.25cm]     (q1) {$$}; 
%         \node[state, right = 0.4cm of q1, accepting] (q2) {$$}; 
%         %\node[state, right of=q2, accepting] (q3) {$$}; 
%         \draw [->] (q1) edge node [above] {\tt $a$} (q2);
%         %\draw [->] (q2) edge node [above] {\tt $b$} (q3);
%       \end{tikzpicture} 
%       \caption*{\hspace{0.5cm}$a$}
%     \end{minipage} 
%     \begin{minipage}[b]{0.18\columnwidth}
%       \centering
%       \begin{tikzpicture}[baseline=-1.80em,initial text=]
%         \tikzstyle{every state}=[inner sep=0pt, minimum size=0.2cm]

%         \node[state, initial, initial distance=0.25cm]     (q1) {$$}; 
%         \node[state, above = 0.3cm of q1] (q2) {$$}; 
%         \node[state, right = 0.3cm of q1, accepting] (q3) {$$}; 
%         \draw [->] (q1) edge node [left] {\tt $a$} (q2);
%         \draw [->] (q2) edge node [above, pos=0.75] {\tt $b$} (q3);
%       \end{tikzpicture} 
%       \caption*{\hspace{0.5cm}$a \cdot b$}
%     \end{minipage} 
%     \begin{minipage}[b]{0.18\columnwidth}
%       \centering
%       \begin{tikzpicture}[baseline=-1.80em,initial text=]
%         \tikzstyle{every state}=[inner sep=0pt, minimum size=0.2cm]

%         \node[state, initial, initial distance=0.25cm]     (q1) {$$}; 
%         \draw (q1) edge[loop above] node [left] {\tt $a$} (q1);
%         \node[state, right = 0.4cm of q1, accepting] (q2) {$$}; 
%         \draw [->] (q1) edge node [above] {\tt $\epsilon$} (q2);
%       \end{tikzpicture} 
%       \caption*{\hspace{0.45cm}$a*$}
%     \end{minipage} 
%     \begin{minipage}[b]{0.18\columnwidth}
%       \centering
%       \begin{tikzpicture}[baseline=0em,initial text=]
%         \tikzstyle{every state}=[inner sep=0pt, minimum size=0.2cm]

%         \node[state, initial, initial distance=0.25cm]     (q1) {$$}; 
%         \node[state, above right = 0.4cm of q1]     (q2) {$$}; 
%         \node[state, below right = 0.4cm of q1]     (q3) {$$}; 
%         \node[state, below right = 0.4cm of q2, accepting]     (q4) {$$}; 
%         \draw [->] (q1) edge node [above, pos=0.25] {\tt $\epsilon$} (q2);
%         \draw [->] (q1) edge node [below, pos=0.25] {\tt $\epsilon$} (q3);
%         \draw [->] (q2) edge node [above, pos=0.75] {\tt $a$} (q4);
%         \draw [->] (q3) edge node [below, pos=0.75] {\tt $b$} (q4);
%       \end{tikzpicture} 
%       \caption*{\hspace{0.6cm}$a \vert b$}
%     \end{minipage} 
%     \hspace{0.02\columnwidth}
%     \vline
%     %\hspace{0.01\columnwidth}
%     \begin{minipage}[b]{0.18\columnwidth}
%       \centering
%       \tikzset{invisible/.style={minimum width=0mm,inner sep=0mm,outer sep=0mm}}
%       \begin{tikzpicture}%[baseline=(current bounding box.north)]
%         [initial text=]
%         \tikzstyle{every state}=[inner sep=0pt, minimum size=0.2cm]

%         % \node[state, initial]     (q1) {$$}; 
%         % \node[state, right of=q1, accepting] (q2) {$$}; 
%         % %\node[state, right of=q2, accepting] (q3) {$$}; 
%         % \draw [->] (q1) edge node [above] {\tt $a$} (q2);
%         % %\draw [->] (q2) edge node [above] {\tt $b$} (q3);

%         \node[state, initial, initial distance=0.25cm] (q1) {$$};
%         %\node[state, right = of q1] (q2) {$q_2$};
%         \node[state, above right = 0.4cm of q1] (q2) {$$};
%         \node[state, below right = 0.4cm of q1] (q3) {$$};
%         \node[state, below right = 0.4cm of q2, accepting] (q4) {$$};

%         \draw[->] (q1) edge [] node [above, pos=0.25] {\tt $\epsilon$} (q2);
%         \draw[->] (q1) edge [] node [below, pos=0.25] {\tt $\epsilon$} (q3);
%         \draw[->] (q2) edge [] node [above, pos=0.75] {\tt $a$} (q4);
%         \draw[->] (q3) edge [] node [below, pos=0.75] {\tt $a$} (q4);

%         \node[label=left:{$\epsilon$}, above= 0.47cm of q1,invisible] (above1) {};
%         \draw (q4) |- (above1);
%         \draw[->] (above1) -- (q1);
%       \end{tikzpicture} 
%       \caption*{\hspace{0.7cm}$(a \vert a)$+}
%     \end{minipage}
%     % \caption{
%     %     \KREsAcro operators and NFA equivalents for character, concatenation, repetition, and disjunction.
%     %     NFAs for \KREsAcros have in-degree and out-degree $\leq 2$, although this is higher under $\epsilon$-closure.
%     %     The final figure shows an exponentially ambiguous \KREsAcro.
%     % }
%     \label{figure:regex2NFA} 
% \end{figure} 

% \begin{table}
%     % DECREASE FONT SIZE?
%     %\scriptsize
%     %\footnotesize
%     %\small
%     \centering
%     \caption{
%       Regexes, time complexity, and the length of problematic input $|w|$ that necessitates a 10-second regex match in \TODO{Java-OpenJDK-X.XX}.
%       Each of these exhibits slow behavior on the input ``a$\stackrel{n}{\cdots}$ab''.
%       Machine is desktop class (\TODO{CPU specs go here}).
%     }
%     \begin{tabular} {cccc}
%     \toprule
%     \textbf{Regex}  & \textbf{Complexity}   & \textbf{$|w|$} \\
%     \toprule
%     \verb<^a*a*$<   & $\mathcal{O}(|w|^2)$  & ? \\
%     \verb<^a*a*a*$< & $\mathcal{O}(|w|^3)$  & ? \\
%     \verb<^(a|a)*$< & $\mathcal{O}(2^{|w|})$ & ? \\
%     \verb<^(a*)*$<  & $\mathcal{O}(2^{|w|})$ & ? \\
%     \bottomrule
%     \label{table:RegexQueryResponseTiming}
%     \end{tabular}
%     \vspace{-0.30cm}
% \end{table} 




==> rw-old.tex <==
%!TEX root = main.tex

\FS{@Adnan, @Zainab, could you please update the related work section? You can start by searching the most relevant papers in google scholar, and checking which other papers cite them.}
\JD{Shortening suggestion: This section is currently covering related work beyond the scope of the title (which is oriented towards the regexes alone, not the rest of the solution landscape). From a ``So much introductory matter'' complaint perspective, we can make this a subsection of II --- ``Background and Related Work'' --- which might help us focus the content.}

Regexes are a ubiquitous tool used in security-sensitive contexts.
Given the importance of regexes, researchers have examined the \REDOS problem from many perspectives.
 % in particular, as well as regex engineering practices more generally.

% \JD{@FS If you want to try it, we could put the defense-in-depth figure here or in the introduction. As we discussed, this figure would illustrate different places to apply these defenses, adapting the ``swiss cheese'' concept to \REDOS.}
% \FS{Dongyoon added a figure in the introduction. I asked him to sync it with the subsections here.}

% \mysection{Studies of \REDOS}

\mysection{Empirical measurements of \REDOS in practice}

Although the \REDOS attack was proposed twenty years ago by Crosby and Wallach~\cite{Crosby2003REDOS,Crosby2003AlgorithmicComplexityAttacks}, researchers have only recently attempted to estimate its impact.
In 2018, Davis \etal reported that SL regexes were present in many popular open-source software modules, and that engineers struggled to repair them~\cite{Davis2018EcosystemREDOS}; 
in 2019 they observed that these regexes displayed super-linear (SL) behavior in the built-in regex engines used in most mainstream programming languages~\cite{Davis2019LinguaFranca,Davis2019RegexGeneralizability}.
Concurrently, Staicu \& Pradel showed that 10\% of Node.js-based web services were vulnerable to \REDOS due to their use of vulnerable npm modules~\cite{Staicu2018REDOS}.

These findings motivated substantial further research into the \REDOS problem.
Web services must process user input (\REDOS condition 3), so researchers have examined infrastructure-level solutions (\REDOS condition 1) and application-level solutions (\REDOS condition 2).

\mysection{Changing the Infrastructure}
\label{sec:changingInfrastructure}

\mysubsection{Changing the regex engine}
There are both classic and more recent alternatives to the exponential-time backtracking regex algorithm.
The earliest published regex matching algorithms, by Brzozowski in 1964~\cite{brzozowski1964derivatives} and Thompson in 1968~\cite{Thompson1968LinearRegexAlgorithm}, offer linear-time guarantees.
There are production-grade implementations of Thompson's approach, notably Google's RE2 regex engine~\cite{Cox2010RE2Implementation} and the engines in Rust~\cite{RustRegexDocs} and Go~\cite{GoRegexDocs}.
Microsoft has considered Brzozowski's approach for .NET~\cite{saarikivi2019symbolic}, as well as deterministic matching strategies~\cite{holik2019succinct,turovnova2020regex}. 
However, these algorithms are difficult to adopt in legacy programming languages, since it does not provide support for non-regular regex features.
Davis \etal presented an alternative approach that preserves the backtracking framework~\cite{Spencer1994RegexEngine}, but reduces the time complexity to linear via memoization~\cite{davis2021using}.
While this approach is sound, it trades space for time and may thus simply exhaust another resource instead.

\mysubsection{Abandoning regexes}
To avoid \REDOS, some advocate alternative approaches to string matching. 
Davis \etal reported that reverting to built-in string functions was a popular \REDOS repair technique~\cite{Davis2018EcosystemREDOS}.
However, regexes exist for a reason --- they concisely express long sequences of string operations.
To safely benefit from expressiveness, the most prominent regex alternative is parsing expression grammars (PEGs)~\cite{ford2004parsing}.
The Rosie Pattern Language simplifies converting regexes into PEGs~\cite{jenningsRPL}.
Although this approach is attractive, technical inertia suggests that regexes are here to stay.

\mysection{Coping With SL Regexes}
\label{sec:coping}

The majority of \REDOS research assumes that SL regexes are already present in a web service, and considers various coping mechanisms.

\mysubsection{Detecting SL Regexes}
Many approaches have been proposed to automatically identify super-linear regexes.
Many researchers statically analyze the NFA of the regex.
Berglund \etal \cite{Berglund2014REDOSTheory} defined a prioritized type of NFA to simulate a backtracking engine in Java and decide if a regex will show SL behavior.
Weideman \etal~\cite{Weideman2016REDOSAmbiguity,Weideman2017StaticExpressions} also use a prioritized NFA and look for IDA in it.
Wustholz \etal~\cite{Wustholz2017Rexploiter}, also look for the IDA pattern in the NFA and compute an attack automaton that produces attack input strings.
Liu \etal~\cite{liu21sp} adds support for modeling and analyzing less common regex features, \eg set operations.

Others statically analyze different representations of the regex.
Kirrage \etal~\cite{Kirrage2013rxxr} analyze an abstract evaluation tree of the regex.
Rathnayake \etal~\cite{Rathnayake2014rxxr2} look for exponential branching in the regex evaluation tree.
Sugiyama \etal~\cite{Sugiyama2014RegexLinearityAnalysis} analyzes the size of a tree transducer for the regex. 
Finally, 
Sulzmann \etal~\cite{Sulzmann2017DerivAmbig} use Brzozowski derivatives to create a finite state transducer to generate parse trees and minimal counter-examples. 

Finally, other approaches apply dynamic analysis to detect SL regexes.
Shen \etal~\cite{Shen2018ReScueGeneticRegexChecker} and McLaughlin \etal~\cite{mclaughlin2022regulator} proposed search algorithms for inputs with super-linear matching time.
The broader category of algorithmic complexity detectors, \eg~\cite{Petsios2017SlowFuzz,wei2018singularity,noller2018badger,meng2018rampart,blair2020hotfuzz}, can also be extended to detect \REDOS.

\mysubsection{Repairing SL Regexes}
Other approaches focus on repairing SL regexes to make then non-SL.
 % researchers have proposed automated approaches to repair existing SL regexes.
These approaches offer trade-offs for the repaired regex, in: semantic similarity, (perceived) readability, and support for uncommon features.
Van der Merwe \etal presented a modified flow algorithm to convert an ambiguous K-regex into an equivalent unambiguous one~\cite{VanDerMerwe2017EvilRegexesHarmless}, with perfect semantic equivalence, but lower readability.
Cody-Kenny \etal proposed evolving a regex towards a higher-performing alternative --- though evaluated on average-case performance, this scheme may also work for worst-case performance~\cite{codykenny17},
supporting uncommon features but with only approximate semantics.
More recently, Li \etal~\cite{li2020flashregex} proposed an approach to repair SL regexes with deterministic regex constraints to avoid regex ambiguity.
% caused by the anti-patterns proposed by Davis \etal\cite{Davis2018EcosystemREDOS}.
This approach uses a human-in-the-loop to provide good examples.
Finally, Claver \etal~\cite{claver2021regis} proposed a synthesis-based approach for repairing SL regexes.


% \JD{The parenthetical remark is easily dismissed by a critical reader, who might say ``well why not apply those tools in your CI pipeline?'' How about an argument based in \emph{comprehension} or \emph{ease of adoption} --- we are teaching fundamental concepts in a digestable way, which complements automatic analyses, help engineers make informed repair decisions, allow human-in-the-loop designs, that kind of thing? But we end up having the same argument at the end of the next subsection. That repetition of the argument makes me wonder if we are not structuring this section appropriately, because we are using the same kind of defense in two places...}
% \JD{Discussion point: Write-then-refactor is more expensive than get-right-the-first-time; the re-architecture may be non-trivial and the NFA-based tools would be hard in this circumstance.}

\mysubsection{Recovering From \REDOS}
After a system containing a \REDOS vulnerability is deployed, it is possible to detect and isolate \REDOS attacks to minimize the damage incurred.
Bai \etal proposed the only \REDOS-specific approach of this kind, applying deep learning to detect attack strings and redirect them to a sandbox~\cite{bai2021runtime}.
More general approaches that consider anomalous resource utilization, \eg time~\cite{davis2018sense}, CPU~\cite{meng2018rampart}, or other resources~\cite{demoulin2019detecting}.



{\color{blue}
% \mysection{Addressing \REDOS during Regex Composition}
\mysection{Characterizing Regexes Vulnerable to \REDOS}
Previous work also tried to characterize what regexes are vulnerable to \REDOS.
% To the extent of our knowledge, only two past approaches (partially) characterize IA regexes in the regex modality.
% While substantial study has been made of dealing with SL regexes \emph{after} they enter a codebase, only two existing approaches (partially) support developers at composition time.
% The philosophy of these approaches is to avoid composing IA regexes in the first place.
}
Davis \etal characterized a set of practitioner anti-patterns to avoid \REDOS, but reported that these have a high false positive rate~\cite{Davis2018EcosystemREDOS}.
 % regex-based anti-patterns that were prescribed without much evidence in reference books and best-practice documents by practitioners, recommended to be used as rules of thumb to avoid infinite ambiguity.
Alternatively, Brabrand \& Thomsen developed theories to identify \emph{un}ambiguous regexes, and treat all other regexes as suspect, including both SL regexes and merely finitely ambiguous (\ie non-vulnerable) regexes~\cite{brabrand2010typed}.

Our proposed work provides important improvements over these two approaches.
In contrast with Brabrand \& Thomsen's, our theory distinguishes between finite and infinite ambiguity, enabling developers to distinguish between likely-unproblematic (non-IA) and problematic (IA) regexes.
In contrast with practitioner-prescribed anti-patterns, we provide a theoretical grounding to formally capture their limitations, and we provide new anti-patterns that provide higher precision and recall capturing IA regexes.



% \FS{Should we skip the paragraph below, and only mention this in the discussion?}
% \DY{Sounds like a good idea.}
% Automated SL regex detection and repair techniques could be adapted for usage during regex composition, to continuously automatically scan and repair regex drafts.
% No study of this approach has been conducted.
% Johnson \etal imply that this scheme may be counterproductive for many engineers, who would find it too invasive~\cite{johnson2013don}.

\iffalse
%Based on previous examinations of developers' use of software checking tools, 
However, 
% many developers may still decide against this option, because, \eg, 
the repaired regexes could be hard to understand, and the tooling continuous automatic modification of their draft regex may interrupt the developers' workflow
Our proposed anti-patterns complement this strategy, to now reach more situations, \ie when developers cannot understand (or trust) automatically-repaired regex drafts. 
% , and when developers prefer to create their own understanding of why the regex is IA and make their own informed decision about how to repair it.
Furthermore, our anti-patterns contribute to educating developers in secure coding, which is an important mission~\cite{gasiba21}.
\fi

% \mysubsection{Addressing \REDOS during Regex Composition}
% Developers wanting to avoid composing IA regexes could apply past characterizations of SL regexes
% Past characterizations of SL regexes have been proposed 
% in terms of their NFA \cite{Berglund2014REDOSTheory,Weideman2016REDOSAmbiguity,Weideman2017StaticExpressions,Wustholz2017Rexploiter,liu21sp}, or in terms of the regex parse tree \cite{Kirrage2013rxxr,Rathnayake2014rxxr2,Sugiyama2014RegexLinearityAnalysis,Sulzmann2017DerivAmbig}.
% However, we aim to help developers asking them to reflect only about the regex itself.
% This is more inclusive --- does not require developers to know additional modalities --- and is likely preferred by most developers --- most use only the IDE representation when composing regexes~\cite{bai2019exploring}.

% The goal of our research is to help engineers design safe regexes.
% Our approach will support engineers to recognize problematic regexes during composition and code review, since it characterizes IA regexes in terms of the regex itself (using regex semantics).
% As we described in \cref{section:ProposedApproach}, 
% our goal is to characterize IA regexes (instead of SL ones) as a way to provide simpler theory and anti-patterns, while still capturing all SL regexes (all SL regexes are IA).
% Our goal is also to characterize IA regexes in the regex modality,
% to reach a wide population of developers (including the many who work regularly with regexes but have no formal training in automata~\cite{Michael2019RegexesAreHard,Donohue2019RegexThesis}) 













% Our approach is most closely related to Brabrand \& Thomsen~\cite{brabrand2010typed}, in that we analyze ambiguity directly using regex semantics.
% Our theoretical contribution extends their approach by distinguishing between finite and infinite ambiguity, enabling us to distinguish between likely-unproblematic and problematic regexes. \JD{Previous sentence uses terms that we should define in the Background section (or use other terms instead.)}
% However, we are unique in our effort to provide trustworthy regex-level anti-patterns that can be applied by engineers without reliance on an external tool.
% \JD{perhaps ``\ul{articulate our theoretical results in} trustworthy regex-level anti-patterns...''}

% Anti-patterns
% \subsection{Characterizations of SL and Ambiguous Regexes}
% The goal of our research is to help engineers design safe regexes.
% To this end, we contribute \emph{regex anti-patterns} to help engineers understand the root causes of super-linear behavior.
% We are not the first to propose regex anti-patterns.

% Davis \etal formulated three regex anti-patterns based on descriptions in regex reference books, but their implementation of these anti-patterns had high false positive rates~\cite{Davis2018EcosystemREDOS}.
% Other researchers have proposed ``regex'' anti-patterns based on an automaton interpretation of a regex, \eg searching for nested graph cycles with overlapping labels~\cite{Weideman2016REDOSAmbiguity,liu21sp,DoesWustholzDoThisImNotSure}.
% It is unclear whether this modality is useful to practitioners, many of whom lack formal training in automata~\cite{Michael2019RegexesAreHard,Donohue2019RegexThesis}.
% We are the first to conduct experiments on the efficacy of regex-based anti-patterns, with anti-patterns grounded in our novel analysis of regex ambiguity rather than after a conversion to automata.

% Anti-patterns
% \subsection{Anti-patterns for SL and Ambiguous Regexes}
% \AH{Please check the following paragraph for comparison with Davis'18}
% Previously, Davis \etal\cite{Davis2018EcosystemREDOS} proposed 3 anti-patterns to detect super-linear behaviour in regexes. But these anti-patterns can only detect infinite ambiguity in the regexes. We improve over these anti-patterns in two ways: 
 % (1) our anti-patterns uses regex based terms rather than nfa based terms to improve readability. \JD{This improvement sounds like a search-and-replace, not a fundamental improvement.}
 % (2) our anti-patterns uses theory to cover the cases those are not covered by Davis \etal~\cite{Davis2018EcosystemREDOS}. 
 % \JD{This sounds like a more meaningful difference. You should double-check what we wrote in~\cite{Davis2018EcosystemREDOS}, but perhaps language like this would work: ``Davis \etal's anti-patterns were derived from practitioner literature and based on common engineering practices. They reported false positives and false negatives, but did not include a theoretical grounding to formally capture the limitations of their patterns.''}


% Our work is complementary to these approaches:
%   (1) our approach provides an explanation in terms of regex semantics, rather than requiring a conversion to finite automata;
%   (2) our approach uses anti-patterns to trade perfect accuracy for ease of adoption, and by the same token does not require engineers to adopt new tools.
% Our approach enables engineers to choose an alternative design for their regexes, rather than fine-tuning an existing design. \JD{Not sure about including the previous sentence, since we don't include that in our experiments.}
